Superintelligence Strategy: Expert Version

Rapid advances in AI are beginning to reshape national security. Destabilizing AI developments could rupture the balance of power and raise the odds of great-power conflict, while widespread proliferation of capable AI hackers and virologists would lower barriers for rogue actors to cause catastrophe. Superintelligence -- AI vastly better than humans at nearly all cognitive tasks -- is now anticipated by AI researchers. Just as nations once developed nuclear strategies to secure their survival, we now need a coherent superintelligence strategy to navigate a new period of transformative change. We introduce the concept of Mutual Assured AI Malfunction (MAIM): a deterrence regime resembling nuclear mutual assured destruction (MAD) where any state's aggressive bid for unilateral AI dominance is met with preventive sabotage by rivals. Given the relative ease of sabotaging a destabilizing AI project -- through interventions ranging from covert cyberattacks to potential kinetic strikes on datacenters -- MAIM already describes the strategic picture AI superpowers find themselves in. Alongside this, states can increase their competitiveness by bolstering their economies and militaries through AI, and they can engage in nonproliferation to rogue actors to keep weaponizable AI capabilities out of their hands. Taken together, the three-part framework of deterrence, nonproliferation, and competitiveness outlines a robust strategy to superintelligence in the years ahead.

==> abridged/1-intro.tex <==
% \vspace*{-3\baselineskip}
\section{Introduction}

From geopolitical conflict to catastrophic misuse, the challenges AI poses are far too broad, and far too serious, for piecemeal measures. What is needed is a comprehensive approach, one that does not shy from the unsettling implications of advanced AI. As with Herman Kahn’s famous analysis of nuclear strategy \cite{kahn1960thermonuclear}, superintelligence strategy requires ``thinking about the unthinkable.'' An effective strategy should draw from a long history of national security policy because superintelligence is inescapably a matter of national security.

% AI is advancing at a pace few foresaw, transforming society and compelling policymakers, technologists, and strategists to confront issues from automation-driven economic shifts to strategic competition. Unlike specialized technological tools, AI spans virtually every sector, including finance, healthcare, and defense. This broad applicability, coupled with its rapid evolution, creates a risk landscape that is expansive and difficult to predict. AI’s dual-use nature---spanning civilian and military applications---magnifies both opportunities and threats.

AI lowers barriers for acts of mass destruction once the exclusive domain of major powers. Individuals armed with an expert-level AI virologist could create novel pathogens, while advanced hacking AIs might target energy grids at a national scale. Defense often lags behind offense in both biology and critical infrastructure, leaving large swaths of civilization vulnerable. The relative security we enjoyed when only nation-states were capable of sophisticated attacks will no longer hold if highly capable AIs can guide extremist cells from plan to execution.

Militaries see in AI the key to a decisive edge, igniting a race to develop capabilities that could overturn existing balances of power. Beyond powering next-generation drones, AI raises the specter of strategic breakthroughs that might upend nuclear deterrence. A superintelligence---if its creators can control it---could conceivably deliver a ``superweapon'' and hand its wielders a strategic monopoly on power \cite{wonderweapons}. Superintelligence is not merely a new weapon, but a way to fast-track all future military innovation. A nation with sole possession of superintelligence might be as overwhelming as the Conquistadors were to the Aztecs. In a winner-take-all race, any hint of a looming superweapon fuels tensions, pushing rivals toward actions that could quickly escalate into open conflict. AI development is fast becoming a matter of survival rather than merely technological ambition.

Another hazard emerges when AI systems can autonomously develop the next generation of AIs. Systems that can fully automate the AI research process could telescope a decade of progress into a year. A fast feedback loop could create an ``intelligence explosion,'' resulting in AIs as uncontainable to us as an adult would be to a group of three-year-olds. Racing countries might forgo human oversight of automated research, since it would slow research from machine speed to human speed. If AI systems outpace the safeguards designed for them, we may accidentally unleash an AI which does not follow a commander's intent.


% AI is advancing at a pace few foresaw, transforming society and compelling policymakers, technologists, and strategists to confront issues from automation-driven economic shifts to strategic competition. Unlike specialized technological tools, AI spans virtually every sector, including finance, healthcare, and defense. This broad applicability, coupled with its rapid evolution, creates a risk landscape that is expansive and difficult to predict. AI’s dual-use nature—spanning civilian and military applications—magnifies both opportunities and threats.

% AI lowers barriers for acts of mass destruction once the exclusive domain of major powers. Individuals armed with an expert-level AI virologist could create novel pathogens, while advanced hacking programs might target energy grids at a national scale. Defense often lags behind offense in both biology and critical infrastructure, leaving large swaths of civilization vulnerable. The relative security we enjoyed when only nation-states were capable of sophisticated attacks will no longer hold if highly capable AIs can guide extremist cells from plan to execution.

% Militaries see in AI the key to a decisive edge, igniting a race to develop capabilities that could overturn existing balances of power. Beyond powering next-generation drones, AI raises the specter of strategic breakthroughs that might upend nuclear deterrence. A superintelligence—if its creators can control it—could conceivably deliver a ``superweapon'' and hand its wielders a strategic monopoly on power. In a winner-take-all race, any hint of a looming superweapon fuels tensions, pushing rivals toward actions that could quickly escalate into open conflict. AI development is fast becoming a matter of survival rather than merely technological ambition.



% To navigate these complexities, many have turned to analogies. AI has been compared to electricity for its general-purpose nature, to traditional software for its economic importance, or to the printing press for its cultural impact. While these comparisons provide useful entry points, they fail to emphasize the grave national security implications of AI. A more productive analogy lies between AI and catastrophic dual-use nuclear, chemical, and biological technologies. Like them, AI will be integral to a nation’s power while posing the potential for mass destruction. A brief examination of the historical parallels between AI and the nuclear age can highlight the gravity of our current situation.

% In 1933, the leading scientist Ernest Rutherford dismissed the notion of harnessing atomic power as ``moonshine.'' The very next day, Leo Szilard read Rutherford’s remarks and sketched the idea of a nuclear chain reaction that ultimately birthed the nuclear age. Eventually figures such as J.\ Robert Oppenheimer recognized the dual nature of their work. Today, AI is at a similar stage. Previously considered science fiction, AI has advanced to the point where machines can learn, adapt, and potentially exceed human intelligence in certain areas. AI experts including Geoffrey Hinton and Yoshua Bengio, pioneers in deep learning, have expressed existential concerns about the technologies they helped create \cite{cais2023}.

% As AI's capabilities are becoming more evident, nations and corporations are heavily investing to gain a strategic advantage. The Manhattan Project, which consumed 0.4\% of the U.S.\ GDP, was driven by the need to develop nuclear capabilities ahead of others. Currently, a similar urgency is evident in the global effort to lead in AI, with investment in AI training doubling every year for nearly the past decade. Several ``AI Manhattan Projects'' aiming to eventually build superintelligence are already underway, financed by many of the most powerful corporations in the world.

% \begin{figure}[b]
%     % \vspace{-10pt}
%     \centering
%     \includegraphics[width=\textwidth]{figures/strategy.pdf}
%     \caption{Effective strategies for managing advanced AI can draw from national security precedents in handling previous potentially catastrophic dual-use technology.}
%     \label{fig:strategy}
%     % \vspace{-10pt}
% \end{figure}

% However, the rapid advancement of AI technologies introduces significant uncertainties for international stability and security. The introduction of nuclear weapons altered international relations, granting influence to those who possessed them and leading to an arms race. The Cuban Missile Crisis highlighted how close the world came to nuclear war. Nuclear annihilation has been avoided thus far despite significant tensions between nuclear states in part through the deterrence principle of Mutual Assured Destruction (MAD), where any nuclear use would provoke an in-kind response. In the AI era, a parallel form of deterrence could emerge---what might be termed ``Mutual Assured AI Malfunction'' (MAIM)---where states' AI projects are constrained by mutual threats of sabotage.


% The risks are not limited to state competition; advanced dual-use technologies can also be exploited by non-state actors. Just as the spread of nuclear capabilities raised concerns about misuse, the availability of AI systems presents new challenges. Malicious actors could use AI to develop weapons of mass destruction or conduct large-scale cyberattacks on critical infrastructure. The accessibility of unsecured or open-weight AI increases these risks, highlighting the need for careful policies and safeguards.

% In the nuclear era, uranium became the linchpin of atomic power. States that secured it could enforce regulations, negotiate treaties, and limit the spread of destructive capabilities. In the realm of AI, computing resources---especially AI chips---have a similar strategic weight, fueling rivalries and shaping geopolitical calculations. This dynamic is evident in places such as Taiwan, central to AI chip production, where rising tensions could have extensive consequences. Nations have a shared interest in controlling access to AI chips to keep them out of the hands of rogue actors, echoing the logic once applied to uranium.

% Despite these challenges, AI offers significant opportunities. Nuclear technology, while introducing the threat of mass destruction, also provided a new energy source that transformed societies. AI has the potential to drive advancements across various sectors, from medical breakthroughs to economic automation. Embracing AI's benefits is important for economic growth and progress in the modern world.


% \begin{wrapfigure}{r}{0.5\textwidth}
%     \vspace{-5pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/compute_over_time.png}
%     \caption{The amount of compute used to create AI models has been increasing exponentially for decades \cite{epoch2023aitrends}.\looseness=-1}
%     \vspace{-10pt}
%     \label{fig:computetime}
% \end{wrapfigure}


% From geopolitical conflict to catastrophic misuse, the challenges AI poses are far too broad, and far too serious, for piecemeal measures. What is needed is a comprehensive approach, one that does not shy from the unsettling implications of advanced AI. As with Herman Kahn’s famous analysis of nuclear strategy \cite{kahn1960thermonuclear}, superintelligence strategy requires ``thinking about the unthinkable.'' Superintelligence is inescapably a matter of national security, and an effective strategy should draw from a long history of national security policy.

% In this paper, we propose such a strategy, emphasizing three key pillars of deterrence, competitiveness, and nonproliferation. We introduce the notion of Mutual Assured AI Malfunction (MAIM), arguing that when states possess common knowledge of the existential importance of AI, they will each act to sabotage rival AI projects that threaten their security. MAIM might be used to create a stable deterrence regime, preventing mutual assured AI destruction from escalating into mutual assured human destruction. Meanwhile, governments which rely exclusively on Taiwan for crucial chips leave themselves vulnerable to crippling disruption if tensions escalate. In order to retain economic and military competitiveness in a shifting landscape, nations must secure domestic supply chains for AI chips and drones. Finally, all nations have a shared interest in nonproliferation efforts to limit the AI capabilities accessible to rogue actors. Through these pillars, states can safeguard their security while opening the door to unprecedented prosperity.

In this paper, we propose a superintelligence strategy emphasizing three key pillars of deterrence, competitiveness, and nonproliferation. We introduce Mutual Assured AI Malfunction (MAIM), arguing that when states possess common knowledge of the national security implications of AI, they will each act to sabotage rival AI projects that threaten their security. MAIM might be used to create a stable deterrence regime, preventing mutual assured AI destruction from escalating into mutual assured human destruction. Meanwhile, governments which rely exclusively on Taiwan for crucial chips leave themselves vulnerable to crippling disruption if tensions escalate. In order to retain economic and military competitiveness in a shifting landscape, nations must secure domestic supply chains for AI chips and drones. Finally, all nations have a shared interest in nonproliferation efforts to limit the AI capabilities accessible to ``rogue actors''---terrorist groups and small pariah states. Through these pillars, states can safeguard their security while opening the door to unprecedented prosperity.

Though this abridged paper describes the core of our strategy, we recommend the comprehensive version of this paper---``\href{https://nationalsecurity.ai}{Superintelligence Strategy: Expert Version}''---for those interested in a more detailed strategic analysis covering a broader range of challenges.

\begin{figure}[t]
    % \vspace{-5pt}
    \vspace{5pt}
    \centering
    \includegraphics[width=\textwidth]{figures/strategy_comp_middle.pdf}
    \caption{Effective strategies for managing advanced AI can draw from national security precedents in handling previous potentially catastrophic dual-use technology.}
    \label{fig:strategy}
    % \vspace{-10pt}
\end{figure}


% In this paper, we propose a strategy drawing from the history of national security, emphasizing three key pillars: deterrence, competitiveness, and nonproliferation. We introduce Mutual Assured AI Malfunction (MAIM), arguing that when states possess common knowledge of the national security implications of AI, they will each act to sabotage rival AI projects that threaten their survival. MAIM might be used to create a stable deterrence regime, preventing mutually assured AI destruction from escalating into mutually assured human destruction. Second, we examine competitiveness through supply chains: nations relying solely on Taiwan for crucial AI chips risk crippling disruption, requiring secure domestic production of AI chips and drones. Third, we explore nonproliferation, where all nations share an interest in limiting AI capabilities accessible to rogue actors. Through these pillars, states can safeguard their security while opening the door to unprecedented prosperity.


% The challenges AI poses are far too broad, and far too serious, for piecemeal measures. What is needed is a comprehensive strategy, one that does not shy from the unsettling implications of advanced AI. As with Herman Kahn's famous analysis of nuclear strategy \cite{kahn1960thermonuclear}, superintelligence strategy requires ``thinking about the unthinkable.'' In this paper, we propose such a strategy.



% We argue that the most effective framework for addressing AI’s challenges is to view it through a national security lens. [Tell them what you'll tell them.] %Drawing on lessons from previous dual-use technologies while tailoring them to the distinct demands of AI can help safeguard against catastrophic misuse, maintain geopolitical stability, and ensure that the broader Western world remains at the forefront. %Meeting these demands will require an honest recognition of the stakes, a commitment to learning from historical precedents, and the flexibility to craft innovative policies and practices.

% say do not make assumptions about AGI near vs far; do not need to buy AGI is near to appreciate this point

% Yet, the analogy has its limits. Unlike traditional WMDs, AI is also a cornerstone of national economic competitiveness. Its development fuels progress across industries, drives productivity, and shapes geopolitical influence. The challenge lies in adapting lessons from WMD governance---such as control, verification, and risk mitigation---while fostering the collaboration and capacity necessary for leadership in the global AI landscape. This requires a strategy that balances security and progress, acknowledging AI as a transformative force that will influence both power and prosperity in the decades ahead.

==> abridged/2-strategies.tex <==
\section{Existing Strategies}

States grappling with terrorist threats, destabilizing weaponization capabilities, and the specter of losing control to AI face difficult choices on how to preserve themselves in a shifting landscape. Against this backdrop, three proposals have gained prominence: the first lifts all restraints on development and dissemination, treating AI like just another computer application; the second envisions a voluntary halt when programs cross a danger threshold, hoping that every great power will collectively stand down; and the third advocates concentrating development in a single, government-led project that seeks a strategic monopoly over the globe. Each path carries its own perils, inviting either malicious use risks, toothless treaties, or a destabilizing bid for dominance. Here we briefly examine these three strategies and highlight their flaws.



\begin{enumerate}
\item \textbf{Hands-off (``Move Fast and Break Things'', or ``YOLO'') Strategy.}
This strategy advocates for no restrictions on AI developers, AI chips, and AI models. Proponents of this strategy insist that the U.S.\ government impose no requirements---including testing for weaponization capabilities---on AI companies, lest it curtail innovation and allow China to win. They likewise oppose export controls on AI chips, claiming such measures would concentrate power and enable a one-world government; in their view, these chips should be sold to whoever can pay, including adversaries. Finally, they encourage that advanced U.S.\ model weights continue to be released openly, arguing that even if China or rogue actors use these AIs, no real security threat arises because, they maintain, AI's capabilities are defense-dominant. From a national security perspective, this is neither a credible nor a coherent strategy.

\item \textbf{Moratorium Strategy.}
The voluntary moratorium strategy proposes halting AI development---either immediately or once certain hazardous capabilities, such as hacking or autonomous operation, are detected. Proponents assume that if an AI model test crosses a hazard threshold, major powers will pause their programs. Yet militaries desire precisely these hazardous capabilities, making reciprocal restraint implausible. Even with a treaty, the absence of verification mechanisms \cite{wasil2024verificationmethodsinternationalai} means the treaty would be toothless; each side, fearing the other’s secret work, would simply continue. Without the threat of force, treaties will be reneged, and some states will pursue an intelligence recursion. This dynamic, reminiscent of prior arms-control dilemmas, renders the voluntary moratorium more an aspiration than a viable plan.

\item \textbf{Monopoly Strategy.}
The Monopoly strategy envisions one project securing a monopoly over advanced AI. A less-cited variant---a CERN for AI reminiscent of the Baruch Plan from the atomic era---suggests an international consortium to lead AI development, but this has gained less policymaker interest. By contrast, the U.S.-China Economic and Security Review Commission \cite{uscc2024} has suggested a more offensive path: a Manhattan Project to build superintelligence. Such a project would invoke the Defense Production Act to channel AI chips into a U.S.\ desert compound staffed by top researchers, a large fraction of whom are necessarily Chinese nationals, with the stated goal of developing superintelligence to gain a strategic monopoly. Yet this facility, easily observed by satellite and vulnerable to preemptive attack, would inevitably raise alarm. China would not sit idle waiting to accept the US's dictates once they achieve superintelligence or wait as they risk a loss of control. The Manhattan Project assumes that rivals will acquiesce to an enduring imbalance or omnicide rather than move to prevent it. What begins as a push for a superweapon and global control risks prompting hostile countermeasures and escalating tensions, thereby undermining the very stability the strategy purports to secure.

\end{enumerate}

\begin{figure}[h]
    % \vspace{-10pt}
    \centering
    \includegraphics[width=\textwidth]{figures/flow_chart_short.pdf}
    \caption{Possible outcomes of a U.S.\ Superintelligence Manhattan Project. An example pathway to Escalation: the U.S.\ Project outpaces China without being maimed, and maintains control of a destabilizing AI project but doesn't achieve superintelligence or a superweapon. Though global power shifts little, Beijing condemns Washington’s bid for strategic monopoly as a severe escalation. The typical outcome of a Superintelligence Manhattan Project is extreme escalation, and omnicide is the worst foreseeable outcome.\looseness=-1}
    \label{fig:flow_chart}
    % \vspace{-10pt}
\end{figure}


Rival states, rogue actors, and the risk of losing control call for more than a single remedy. We propose three interconnected lines of effort. First, \emph{deterrence}: a standoff akin to the nuclear stalemate of MAD, in which no power can gamble human security on an unbridled grab for dominance without expecting disabling sabotage. Next, \emph{nonproliferation}: just as fissile materials, chemical precursors, and biological agents have long been denied to terrorists by great powers, AI chips and weaponizable AI systems can similarly be kept from rogue actors. Finally, \emph{competitiveness}: states can protect their economic and military power through a variety of measures including legal guardrails for AI agents and domestic AI chip and drone manufacturing. Our superintelligence strategy, the \textbf{Multipolar Strategy}, echoes the Cold War framework of deterrence, nonproliferation, and containment, adapted to AI’s unique challenges.\looseness=-1

==> abridged/3-maim.tex <==
% \chapter{State Survival}
\section{Deterrence with Mutual Assured AI Malfunction (MAIM)}


In the nuclear age, an initial pursuit of monopoly---one nation seeking unchallenged command of nuclear weapons---eventually gave way to the standoff of deterrence known as mutual assured destruction (MAD). As nuclear arsenals matured and the capability for mutual destruction became undeniable, nations eventually accepted that any bold attempt to dominate all opposition risked drawing a preemptive strike. A similar state of mutual strategic vulnerability looms in AI. If a rival state races toward a strategic monopoly, states will not sit by quietly. If the rival state loses control, survival is threatened; alternatively, if the rival state retains control and the AI is powerful, survival is threatened. A rival with a vastly more powerful AI would amount to a severe national security emergency, so superpowers will not accept a large disadvantage in AI capabilities. Rather than wait for a rival to weaponize a superintelligence against them, states will act to disable threatening AI projects, producing a deterrence dynamic that might be called Mutual Assured AI Malfunction, or MAIM.

\subsection{MAIM Is the Default Regime}
\paragraph{Paths to Disabling a Rival's AI Project.} States intent on blocking an AI-enabled strategic monopoly can employ an array of tactics, beginning with \emph{espionage}, in which intelligence agencies quietly obtain details about a rival’s AI projects. Knowing what to target, they may undertake \emph{covert sabotage}: well-placed or extorted insiders can tamper with model weights or training data or AI chip fabrication facilities, while hackers quietly degrade the training process so that an AI’s performance when it completes training is lackluster. This is akin to Stuxnet which aimed to covertly sabotage Iran's nuclear enrichment program. When subtlety proves too constraining, competitors may escalate to \emph{overt cyberattacks}, targeting datacenter chip-cooling systems or nearby power plants in a way that directly---if visibly---disrupts development. Should these measures falter, some leaders may contemplate \emph{kinetic attacks} on datacenters, arguing that allowing one actor to risk dominating or destroying the world are graver dangers, though kinetic attacks are likely unnecessary. Finally, under dire circumstances, states may resort to \emph{broader hostilities} by climbing up existing escalation ladders or threatening non-AI assets. We refer to attacks against rival AI projects as ``maiming attacks.''

\paragraph{Infeasibility of Preventing Maiming.} Since above-ground datacenters cannot currently be defended from hypersonic missiles, a state seeking to protect its AI-enabled strategic monopoly project might attempt to bury datacenters deep underground to shield them. In practice, the costs and timelines are daunting, and vulnerabilities remain. Construction timelines can stretch to three to five times longer than standard datacenter builds, amounting to several additional years. Costs balloon as well, diverting funds away from the project’s AI chips and pushing total expenditures into the several hundreds of billions. Cooling the world’s largest supercomputer underground introduces complex engineering challenges that go well beyond what is required for smaller underground setups. Should the supercomputer require an order-of-magnitude AI chip expansion, retrofitting the facility would become prohibitively difficult. Even those with the wealth and foresight to pursue this route would still face the potent risks of insider threats and hacking. In addition, the entire project could be sabotaged during the lengthy construction phase. Last, states could threaten non-AI assets to deter the project long before it goes online.

\begin{figure}[t]
    % \vspace{-10pt}
    \centering
    \includegraphics[width=\textwidth]{figures/mad_maim.pdf}
    \caption{The strategic stability of MAIM can be paralleled with Mutual Assured Destruction (MAD). Note MAIM does not displace MAD but characterizes an additional shared vulnerability. Once MAIM is common knowledge, MAD and MAIM can both describe the current strategic situation between superpowers.\looseness=-1}
    \label{fig:mad_maim}
    \vspace{-10pt}
\end{figure}

\paragraph{MAIM Is the Default.} The relative ease of (cyber) espionage and sabotage of a rival’s destabilizing AI project yields a form of deterrence. Much like nuclear rivals concluded that attacking first could trigger their own destruction, states seeking an AI monopoly while risking a loss of control must assume competitors will maim their project before it nears completion. A state can expect its AI project to be disabled if \textit{any} rival believes it poses an unacceptable risk. This dynamic stabilizes the strategic landscape without lengthy treaty negotiations---all that is necessary is that states collectively recognize their strategic situation. The net effect may be a stalemate that postpones the emergence of superintelligence, curtails many loss of control scenarios, and undercuts efforts to secure a strategic monopoly, much as mutual assured destruction once restrained the nuclear arms race.

\subsection{How to Maintain a MAIM Regime}

States eventually came to accept that mutual deterrence, while seemingly a natural byproduct of nuclear stockpiling, demanded deliberate maintenance. Each superpower recognized that advanced defensive measures---particularly anti-ballistic missile (ABM) systems---could unravel the fragile balance that restrained either side from a catastrophic first strike. They responded by safeguarding mutual vulnerabilities, culminating in the 1972 ABM Treaty. By analogy, we should not leave to chance today’s default condition of MAIM: where would-be monopolists, gambling not to cause omnicide, can expect their projects to be disabled. Even if attempting to harden massive datacenters is extraordinarily prohibitive and unwise, rumors alone can spark fears that a rival is going to risk national security and human security. Formal understandings not to pursue such fortifications help keep the standoff steady. We now discuss additional measures that curb unintended escalation and limit collateral damage, so that MAIM does not unravel into broader conflict.

\paragraph{Preserve Rational Decision-Making.} Just as nuclear rivals once mapped each rung on the path to a launch to limit misunderstandings, AI powers must \emph{clarify the escalation ladder} of espionage, covert sabotage, overt cyberattacks, possible kinetic strikes, and so on. For deterrence to hold, each side's readiness to maim must be common knowledge, ensuring that any maiming act---such as a cyberattack---cannot be misread and cause needless escalation. However, clarity about escalation holds little deterrence value if rogue regimes or extremist factions acquire large troves of AI chips. Measures to \emph{prevent smuggling} of AI chips keep decisions in the hands of more responsible states rather than rogue actors, which helps preserve MAIM's deterrent value. Like MAD, MAIM requires that destabilizing AI capabilities be restricted to rational actors.

\paragraph{Expand the Arsenal of AI Project Cyberattacks.} To avoid resorting to kinetic attacks, states could improve their ability to maim destabilizing AI projects with cyberattacks. They could identify AI developers' projects or collect information on the professional activities of AI developers' scientists. To spy on AI projects at most companies, all that is necessary is a Slack or iPhone zero-day software exploit. States could also poison data, corrupt model weights and gradients, disrupt software that handles faulty GPUs, or undermine cooling or power systems. Training runs are non-deterministic and their outcomes are difficult to predict even without bugs, providing cover to many cyberattacks. Unlike kinetic attacks, some of these attacks leave few overt signs of intrusion, yet they can severely disrupt destabilizing AI projects with minimal diplomatic fallout. %The specter of sabotage presses any actor seeking a runaway AI monopoly to reckon with the risk of project ruin before it ever reaches completion.

\begin{wrapfigure}{r}{0.4\textwidth}
\centering
\vspace{-5pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|>{\centering\arraybackslash}p{0.95\linewidth}|}
Large scale attack on many datacenters; threatening non-AI-related assets \\ 
\hline
\emph{Escalation to Broader Hostilities} \\ 
\hline
Kinetic attacks on datacenters or corresponding power plants \\ 
\hline
\emph{Kinetic Threshold} \\ 
\hline
Cyberattacks on datacenters or corresponding power plants; deleting code\\ 
\hline
\emph{Overt Sabotage Threshold} \\ 
\hline
Model weights stolen;  covert attacks to degrade training runs of destabilizing AI projects; cyberattacks causing GPUs to fail more often \\ 
\hline
\emph{Covert Sabotage Threshold} \\ 
\hline
Espionage of AI developer workspace communications, personnel devices, and facilities\\ 
\end{tabular}
\caption{An example MAIM escalation ladder with maiming actions.}
\label{tab:ai_escalation_ladder}
\vspace{-30pt}
\end{wrapfigure}

\paragraph{Build Datacenters in Remote Locations.} During the nuclear era, superpowers intentionally placed missile silos and command facilities far from major population centers. This principle of \emph{city avoidance} would, by analogy, advise placing large AI datacenters in remote areas. If an aggressive maiming action ever occurs, that action would not put cities into the crossfire.

\paragraph{Distinguish Between Destabilizing AI Projects and Acceptable Use.} 
The threat of a maiming attack gives states the leverage to demand transparency measures from rivals, such as inspection, so they need not rely on espionage alone to decide whether maiming is justified. Coordinating can help states reduce the risk of maiming datacenters that merely run consumer-facing AI services. The approach of mutual observation echoes the spirit of the Open Skies Treaty, which employed unarmed overflights to demonstrate that neither side was hiding missile deployments. In a similar spirit, increased transparency spares the broader ecosystem of everyday AI services and lowers the risk of blanket sabotage.

%States may even demand limited inspections or transparency commitments from these facilities---backed by the threat of maiming---to verify they are not clandestinely developing destabilizing capabilities.


\paragraph{AI-Assisted Inspections.} Speculative but increasingly plausible, confidentiality-preserving AI verifiers offer a path to confirming that AI projects abide by declared constraints without revealing proprietary code or classified material. By analyzing code and commands on-site, AIs could issue a confidentiality-preserving report or simple compliance verdict, potentially revealing nothing beyond whether the facility is creating new destabilizing models. Humans cannot perform the same role as easily, given the danger of inadvertently gleaning or leaking information, so AIs could reshape the classic tension between security and transparency \cite{COE_VAYNMAN_2020}. Information from these AI inspections could help keep any prospective conflict confined to the disabling of AI development programs rather than escalating to the annihilation of populations. Such a mechanism can help in the far future when AI development requires less centralization or requires fewer computational resources.

MAIM can be made more stable with unilateral intelligence gathering (espionage), multilateral intelligence gathering (verification), unilateral maiming (sabotage), and multilateral maiming (joint off-switches). Mutual assured AI malfunction, under these conditions, need not devolve into mutual assured human destruction.\looseness=-1


A standoff of destabilizing AI projects may arise by default, but it is not meant to persist for decades or serve as an indefinite stalemate. During the standoff, states seeking the benefits from creating a more capable AI have an incentive to improve transparency and adopt verification measures \cite{scher2024mechanisms}, thereby reducing the risk of sabotage or preemptive attacks. In the Conclusion, we illustrate how this standoff might end, allowing AI’s benefits to grow without global destabilization.

% In the pages ahead, we discuss how these checks could be established and what transitions beyond MAIM might entail. Such measures can ease tensions, allow more ambitious AI endeavors, and curb destabilizing arms-race dynamics. MAIM, while stabilizing, is no permanent fixture, and the conclusion explores how it might ultimately be left behind.


% should say this doesn't matter if it happens extremely fast or extremely slow
% add thing about how this isn't a multidecade strategy; way out of this state described in the conclusion

% The qualification that massively increasing amounts of compute are needed for frontier models, even if copycats need less compute. Probably also good to hedge by saying that if we eventually discover ways to use very little compute for training, or if distributed training works really well, this would make MAIM much harder to maintain




% Note all the ways how it’s not a technical problem; ir not technical; malicious use runs through open weight not technical;










% revise first and last sentences
% We draw on historical lessons to address the unique challenges posed by advanced artificial intelligence. By focusing on creating compute security, increasing information security, and adding AI safeguards, we tackle critical points in the AI pipeline: controlling access to powerful computational resources, protecting sensitive information, and bolstering AI systems against malicious use. Each section offers strategies that, together, form a comprehensive approach to managing risks without markedly hindering AI development.

% Our method relies on layered defenses rather than striving for absolute certainty through provable guarantees. Seeking mathematical assurances of complete security for AI chips, computer systems, and AI systems can be impractical and restrictive. Instead, we accept that no single measure can address every vulnerability and recommend implementing multiple security measures. For the compute security, we recommended record-keeping, tamper-evident cameras, geolocation features, and more. In information security, we recommended multi-factor authentication, the principle of least privilege, insider threat programs, and more. For AI safeguards, we recommended output filters, know-your-customer protocols, mandatory testing, and more.

% By integrating these layers, we build a resilient framework capable of adapting to emerging threats. This defense-in-depth strategy acknowledges that while no individual measure is foolproof, their combination offers substantial security. In doing so, we provide a practical roadmap to prevent advanced AI systems from unintentionally becoming weapons of mass destruction.


% should mention we primarily focused on terrorism for restricting capabilities; MAIM is the main way to deal with states like China in the shorter term

% first is intent, latter three are capabilities.

% Drawing lessons from the WMD Playbook---export controls, information security, domestic safeguards, and verification regimes---we present a playbook tailored to AI.

==> abridged/4-competitiveness.tex <==
\section{Competitiveness}

Although deterrence may prevent destabilizing AI projects, competitiveness remains a decisive factor, and nowhere is this more evident than in the looming risk of a Chinese invasion of Taiwan. Multiple assessments now place the probability of a Chinese invasion or blockade in the double digits within this decade. Such a conflict would carry enormous stakes for the West: Taiwan’s semiconductor fabrication plants are the source of the advanced AI chips outside China. A blockade or invasion would instantly deprive the West of AI chips, eliminating its primary edge in AI. China, having poured resources into domestic chip manufacturing for years \cite{reuters2024china}, would be better insulated from this shock, while many Western nations have hesitated to build or subsidize new foundries at home. Worse, on the battlefield, China’s lead in drone technologies would pose a second challenge, introducing a cheap and agile weapon system against which Western forces are not fully prepared. These events could potentially vault China ahead economically and militarily and become a unipolar force.

These vulnerabilities must be addressed before they become crises. Economic strength depends on securing access to AI chips and ending sole-source dependence on one of the world’s most volatile regions. Military strength requires that states rapidly scale up drone manufacturing. By expanding and securing supply chains for AI chips and drones, governments can ensure that competitiveness is not lost the instant a single pillar---Taiwan---topples.


\subsection{Economic Strength}

\begin{wrapfigure}{r}{0.4\textwidth}
    \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{figures/taiwan.pdf}
    \caption{A Chinese invasion of Taiwan would remove the West's access to new AI chips.\looseness=-1}
    \vspace{-10pt}
    \label{fig:taiwan}
\end{wrapfigure}

\paragraph{AI Chips as the Currency of Economic Power.} As AI becomes more deeply integrated in the economy, the possession of advanced AI chips may define national power. Historically, wealth and population size underpinned a state's influence; however, the automation of tasks through AI alters this dynamic. A collection of highly capable AI agents, operating tirelessly and efficiently, rivals a skilled workforce, effectively turning capital into labor. In this new paradigm, power will depend both on the capability of AI systems and the number of AI chips on which they operate. Nations with greater access to AI chips could outcompete others economically. This shift raises the stakes for any disruption to AI chip supplies.
An invasion of Taiwan, always a concern, could become more tempting for China if its leaders conclude that shutting down Taiwan’s semiconductor production would cripple Western AI capabilities.


\paragraph{Create a Secure AI Chip Supply Chain.} To guard against this vulnerability, nations could invest in building advanced AI chip fabrication facilities within their own borders and reinforce a more resilient supply chain. Constructing such facilities domestically entails higher costs---over 30\% more than in Taiwan---but government subsidies can bridge this gap. This effort is urgent because fabrication facilities take years to become operational.

This strategic move mirrors historical efforts to control critical technologies. During the Manhattan Project, significant investment was made not only in the development of nuclear weapons at Los Alamos but also in uranium enrichment at Oak Ridge. Similarly, ensuring access to AI chips requires substantial investment in both innovation and manufacturing infrastructure. By making the AI chip supply chain more robust, states can prevent a foreseeable devastating defeat.



\subsection{Military Strength}

Even if a state pioneers a breakthrough, it risks falling behind if it fails to integrate that capability into real-world operations \cite{horowitz2010diffusion}. Britain introduced the first tanks during World War I but was soon eclipsed by Germany’s systematic adoption of tanks in the second World War. We turn next to three short-term imperatives for AI diffusion in the military: securing a reliable drone supply chain, carefully weaving AI into command and control, and integrating AI into cyber offense.

\paragraph{Secure Drone Supply Chains.} Although general-purpose AI can pose larger-scale dangers, drones occupy a more conventional yet increasingly pivotal role on modern battlefields \cite{Pettyjohn2024Swarms, unmannedaerial}. Drones are cheap, agile, lethal, and decentralized, attributes that make them indispensable for states determined to keep pace with military trends. Yet many states remain heavily reliant on Chinese manufacturers for key drone and robotics components, leaving them vulnerable if those parts are withheld or disrupted at a decisive juncture.

\paragraph{Diffuse AI Into Command and Control and Cyber Offense.}
Modern battlefields demand rapid decisions drawn from torrents of data across land, sea, air, and cyber domains. AI systems can sift through these streams faster than human officers, enticing commanders to rely on automated judgments. Similarly, AI hacking systems which outpace humans in speed and cost could greatly expand a military's capacity to perform cyberattacks.

Incorporating AI into command and control and cyberoffense would significantly enhance military capabilities, yet this dynamic risks reducing ``human in the loop'' to a reflexive click of ``accept, accept, accept,'' with meaningful oversight overshadowed by the speed of events. Demanding human approval of all individual lower-level engagements may be less important than ensuring explicit human approval for more severe or escalatory attacks. However, human oversight of key military decisions is nonetheless crucial. A human backstop can reduce the risk of a ``flash war'' \cite{hendrycks2023overviewcatastrophicairisks}, akin to the 2010 flash crash \cite{vaughan2020flash}, where a minor AI mistake might spiral into destructive reprisals before any human can intervene.

\paragraph{}

By securing and expanding AI chip and drone supplies, states can safeguard their economic and military competitiveness. AI and an invasion of Taiwan are poised to reshape global power dynamics. Those who fail to act decisively will find themselves at the mercy of those who do.

% The AI revolution is already reshaping global power. Those who do not act decisively will find themselves at the mercy of those who do.




% \subsection{Create a Compute Suppliers Group}

% In the Compute Security section, we discussed reliably knowing where AI chips are and preventing them from falling into the hands of rogue actors. Such measures benefit any state that adopts them. Yet states seeking to strengthen their relative position may choose to be aggressive and consider how to deprive strategic competitors of the means to catch up. Limiting shipments of finished AI chips alone does not stop strategic competitors. States may consider being less cooperative and limit access to the equipment and materials that enable rivals to fabricate their own chips. A ``Compute Suppliers Group'' \cite{zelikow2024defense}, modeled on the precedents of the Nuclear Suppliers Group and the Australia Group, would form a group of governments that control pivotal bottlenecks in the semiconductor supply chain.

% \paragraph{Controlling the Export of Semiconductor Tools and Materials.}  The production of AI chips involves a complex and specialized supply chain with critical choke points. Many essential components are produced by single suppliers, and disruption at any of these points would halt production. ASML in the Netherlands holds a monopoly on advanced extreme ultraviolet (EUV) lithography machines essential for cutting-edge chip fabrication. TSMC in Taiwan accounts for over 90\% of the global market share in advanced semiconductor manufacturing processes below 10 nanometers. Unique resources like the quartz crucibles from Spruce Pine, North Carolina, are vital for producing the high-purity silicon crystals used to make chips.

% Approximately 90\% of the value added in the compute supply chain resides within allied nations, including the United States, the Netherlands, the UK, South Korea, Taiwan, and others \cite{khan2021semiconductor}. This concentration presents a strategic opportunity to control the export of semiconductor manufacturing tools and obstruct strategic competitors from independently producing advanced AI chips. By aligning export policies, sharing intelligence on suspicious activities, and coordinating enforcement, these suppliers would create a unified block against the unauthorized proliferation of semiconductor tools.

% \paragraph{Chips for Peace.} A more ambitious proposal is to go beyond a Compute Suppliers Group and create a ``Compute Coalition'' that mirrors ``Atoms for Peace,'' President Eisenhower’s initiative that offered nuclear technology to participating nations under the condition of strict oversight. In a ``Chips for Peace'' \cite{OKeefe2024} approach, member states would gain privileged access to high-end AI chips and the key components that enable their manufacture. In exchange, they would pledge to secure those chips, maintain declared datacenters subject to inspections, and install AI safeguards against terrorist use and loss of control hazards. This arrangement could serve as both carrot and stick: non-member states risk falling behind and losing economic competitiveness if they choose not to participate.

% \paragraph{China Membership.} China’s willingness to join would likely hinge on which factors most influence AI capabilities. There are many axes which affect AI capabilities: algorithms, data, compute, energy, and diffusion. The U.S.\ and China are roughly tied on algorithms and data, as both have access to the same research papers and both can scrape the internet for data. However, China has an edge on energy production and arguably diffusion, owing to its top-down structure. In contrast, the U.S.'s main advantage is compute. If this edge proves durable, China may try to participate in a Compute Suppliers Group. Should China choose not to join the group, it still has strong incentives to implement compute security measures independently. Unauthorized use and proliferation of AI chips present significant national security risks, including the potential for increased terrorist capabilities. Absent cooperation, China would do well to know where its AI chips are and stem smuggling to rogue actors.


% \subsection{Facilitate Immigration for AI Scientists}
% %American leadership in AI depends, in part, on attracting exceptional researchers from abroad. 
% Just as the United States once harnessed the talents of immigrant scientists during the Manhattan Project, so too does American leadership in AI partly rely on attracting exceptional AI scientists from abroad. In a recent survey, 60\% of non-citizen AI PhDs working in the United States reported significant immigration difficulties, and many indicated that these challenges made them more likely to leave \cite{Aiken2020}. As global competition for AI talent intensifies, implementing reliable immigration pathways tailored specifically to AI scientists will help ensure that the United States remains at the forefront of AI development. By refining visa and residency policies for these researchers---distinct from broader immigration reforms and southern border policy---the United States can maintain its edge in an area increasingly vital to both national security and economic strength.


% \section{Legal Frameworks Governing AI Agents}
% % this section needs better sign posting

% Because AI is so new, our legal frameworks have not yet adapted to the challenges it presents. We must devise new ways to regulate the behavior of AI systems that act with a measure of autonomy. As AI becomes deployed through the economy, it is imperative to establish legal structures to govern AI assistants or AI agents. These structures must balance the need for innovation with the necessity of preventing harm, without imposing overly restrictive measures that could hinder economic security and thereby national security.

% \subsection{Aligning Individual AI Agents}
% Ethical dilemmas have long been subjects of intense debate, with no definitive resolutions in sight. Yet, in the absence of universal answers to what individuals ought to do, societies have crafted legal systems to punish unacceptable behaviors and promote safety and prosperity. While no legal system is perfect, many share foundational principles that generally function effectively. For instance, laws prohibit murder, governments enforce contracts, and those who cause harm are often required to provide restitution. Legal frameworks are not intended to ensure optimal behavior from all; such an endeavor would unduly constrain individual liberties and prove ineffective. However, they deter some of the worst actions, leaving society to use informal institutions and economic incentives to encourage beneficial conduct. %employ social and interpersonal methods to encourage beneficial conduct.

% We contend that the same principles will apply to AI. Determining a universal solution for AI behavior in all scenarios is intractable. Yet, we need not postpone legislating AI behavior until every question about AI values is resolved. Rather, we can start formulating principles to govern AI conduct and prevent harmful actions, without unduly limiting the functions of various AIs.

% While existing laws are not entirely sufficient for governing AI---especially since many laws rely on human intent and mental states---we can adapt legal concepts to establish constraints for AI agents so that they follow the spirit of the law.
% In particular, though much law hinges on the mindset or intention behind an act (\textit{mens rea}), we can ensure that AI does not carry out the acts (\textit{actus reus}) the law is meant to prohibit.
% %In particular, while much of the law is about \textit{mens rea}, we can have AIs refrain from the \textit{actus reus} that a legal prohibition aims to prevent.
% Further, by treating AI as assistants to human principals, we can impose constraints that mirror those already applied to human behavior, ensuring that AI agents contribute positively to society without causing undue harm.

% \subsubsection{Constraints on AI Behavior}

% We propose some basic constraints on AI behavior similar to human legal obligations, including obligations to the public like preventing harm and not lying, and special obligations to the AI's human principal.

% \paragraph{Duty of Care to the Public (Reasonable Care).} AI agents should exercise a level of caution commensurate with that of a reasonable person in similar circumstances to prevent harm. This is the legal concept of \emph{reasonable care}. This involves avoiding actions that could foreseeably cause harm in a legal sense---such as violating tort or criminal laws---rather than merely offending sensibilities or engaging in controversial discourse. The application of reasonable care is context-dependent; for instance, providing detailed information about weapons materials might be appropriate for a verified professional but not for an unvetted individual.

% \paragraph{Duty Not to Lie.} AI agents should refrain from making statements they know to be false. This would be overly restrictive for humans, who are allowed to lie to one another in most situations, but chilling effects on free speech are less relevant for AIs. Moreover, since AIs can be tested, it is more feasible to determine whether an AI overtly lied than it is with humans. Instead, they should be held to a standard more similar to the prohibitions against perjury and fraud even in casual or professional settings. This is separate from nuances like puffery or strategic omissions. AI agents should avoid overt lies, opting instead to withhold responses when necessary. 

% \paragraph{Duty of Care to the Principal (Fiduciary Duties).} In their role as assistants, AI agents owe special obligations to their principals. They should act with loyalty, prioritizing the principal's interests without engaging in self-dealing or serving conflicting interests simultaneously. Additionally, they should keep the principal \textit{reasonably informed}, providing pertinent information without key omissions to enable informed consent.

% \subsubsection{Custom Goals and Market-Driven Variations}
% Within these legally inspired constraints, there is ample room for diversity in how AI agents are designed and operate. The free market and consumer preferences can shape the specific goals and propensities of AI agents. Some may prioritize speed and efficiency, delivering quick results with minimal embellishment, while others might focus on providing thorough, well-crafted responses. Personality traits---such as humor, formality, or reservedness---can also be tailored to suit different user preferences and contexts. For example, a customer support AI might be programmed to avoid discussions on irrelevant topics, maintaining focus on service-related issues. This customization allows AI agents to meet the varied needs of users across different industries and personal preferences. 

% % \subsubsection{Aligning AI Value Systems}

% % AI agents inherently possess value systems that influence how they accomplish goals. These value systems often emerge from their initial training data and can inadvertently reflect biases---such as a tendency toward certain political leanings---that were not explicitly programmed. To address this, we can implement strategies to align AI value systems more deliberately.

% % \paragraph{Alignment with Societal Values.} One method is to align AI agents with the collective preferences of a citizens' assembly. By incorporating the values expressed through deliberation and voting, AI agents can reflect a more representative and democratically informed set of values. This approach fuses multiple moral perspectives, leading to AI behavior that aligns with societal norms. Regular updates can keep the AI in sync with evolving values.

% % \paragraph{Alignment with Individual Preferences.} Alternatively, AI agents can be customized to mirror the values of individual users. This personalization allows the AI to reflect the user's ethical beliefs, political orientations, and stylistic choices. For instance, an AI assistant for a vegetarian user would recognize and support the user's dietary choices in its recommendations. However, alignment should be contextually appropriate; an AI cannot adopt preferences irrelevant to its nature, such as desiring physical experiences.

% % \paragraph{Alignment with Individual Preferences.} Instead of aligning all AI agents with a single set of societal values determined by a citizens' assembly, we could also customize \emph{each} AI to match the values of its individual user. For example, an AI assistant for a conservative user would support conservative policies, while one for a progressive user would endorse progressive positions. % However, this personalization should be appropriate to the AI's nature and capabilities. For instance, while a user may value drinking water, the AI should not value drinking water for itself; the AI cannot adopt preferences that are nonsensical for it to have as a machine.

% \paragraph{}
% Grounding AI behavior in legal principles offers a pragmatic framework for governing AI agents, ensuring they act in ways that prevent harm and uphold societal standards. Within these boundaries, customization and market dynamics can shape the specific characteristics of AI agents, allowing for diversity and innovation. % Aligning AI value systems---whether through societal consensus or individual preferences---further refines their behavior, enhancing trust and effectiveness in their interactions.
% This approach avoids the pitfalls of imposing narrow or arbitrary ethical standards. By leveraging established legal concepts and societal processes, we can shape AI actions in a manner that respects individual freedoms and fosters a pluralistic environment where AI contributes positively to society without undue restrictions.



% \subsection{Aligning Collectives of AI Agents}
% The emerging presence of AI agents online will soon result in a complex ecosystem where these entities execute tasks for users, conduct financial transactions, handle sensitive information, and enter into contracts---often engaging with a multitude of other agents and systems. This proliferation poses significant challenges: when interacting with an AI agent, one may remain unaware of where it operates, the entities behind its deployment, or its history of conduct. Should an agent cause harm, pursuing legal remedy becomes an arduous endeavor.

% \paragraph{Establishing Trust Mechanisms and Institutions.} To navigate these challenges, we must develop mechanisms that reinforce trust and accountability within the network of AI agents. \emph{Insurance services} can underwrite the risks inherent in agent interactions, providing a safeguard against potential losses. By transferring liability from users and developers to insurers, these services enable broader participation in the agent ecosystem while mitigating financial risks. \emph{Action firewall services} can oversee and regulate agent activities, acting as intermediaries that filter and monitor actions initiated by AI agents. They ensure that agents adhere to legal and ethical standards, thereby fostering trust among parties that interact with them. \emph{Reputation systems} can chronicle and disseminate information regarding agent behavior, enabling parties to assess the reliability of agents they engage with. By maintaining records of past interactions and outcomes, these systems help identify agents that consistently act in good faith. \emph{Mediation and collateral arrangements} offer further security, wherein disputes are resolved through impartial entities, and agents furnish guarantees against misconduct. By requiring agents to provide collateral, parties gain assurance of compensation in case of breach, while mediation services facilitate fair resolutions.

% \paragraph{Linking AI Agents to Human Legal Entities via IDs.} A foundational measure involves assigning unique identifiers to AI agents, anchoring them to human-backed legal entities. This linkage ensures that agents do not operate in anonymity and that lines of accountability are distinctly drawn. It should become customary that AI agents abstain from providing services or exchanging resources with other agents not connected to legitimate legal entities---entities not solely backed by AI agents themselves.

% \paragraph{Deferring Consideration of AI Rights.} It is imperative to clarify that this approach does not entail granting rights or direct accountability to AI agents themselves. Bestowing rights upon AI agents presents ambiguous benefits at best, with clear and significant downsides. An AI agent can be replicated and deployed in mere seconds, whereas cultivating a human being to maturity demands decades. Granting rights to AI could lead to a rapid proliferation of autonomous entities that outpace human control. Moreover, heightened intelligence in AI does not inherently equate to moral discernment; history records many intelligent individuals who act without ethical consideration. Since we are unlikely to attain definitive certainty about AI consciousness in the near term, it is prudent to postpone the consideration of AI rights. By deferring this decision, we avoid the risks associated with prematurely granting rights to entities whose moral status remains uncertain.


% By instituting legal frameworks and cultivating institutional mechanisms, we can avert the emergence of a chaotic AI ecosystem. Tethering AI agents to human-backed legal entities and implementing systems that enhance accountability and trust positions us to adeptly manage the complexities introduced by the widespread deployment of AI agents.


% \begin{figure}[h]
% \hspace{-46pt}
% \begin{booktabs}{
%   colspec={p{4.56cm} p{4.2cm} p{4.2cm} p{4.2cm}}, % Adjust widths as needed
%   % colspec={llll},
%   row{odd}={blue9},
%   row{1}={white}
% }
% \toprule
%  & \textbf{Low Control} & \textbf{Medium Control} & \textbf{High Control} \\
% \midrule

%  \begin{tabular}{@{}l@{}}\textbf{Risk Management}\end{tabular} 

%  & Accelerate---no restrictions 
%  & \begin{tabular}{@{}l@{}}Deterrence with MAIM\\Nonproliferation\\Competitiveness\end{tabular} 
%  & Pause AI \\

% \begin{tabular}{@{}l@{}}\textbf{Distribution of Cutting-Edge}\\\textbf{AI Weights Among States}\end{tabular}

%  &  \begin{tabular}{@{}l@{}}Everyone including\\rogue states (open weight)\end{tabular} 
%  & \begin{tabular}{@{}l@{}}Multipolar regime with\\responsible states\end{tabular} 
%  & \begin{tabular}{@{}l@{}}Unipolar regime with\\strategic monopoly\\(AI Manhattan Project)\end{tabular} \\

% \begin{tabular}{@{}l@{}}\textbf{Government Control}\\\textbf{over Domestic AI}\end{tabular}
%  & No involvement 
%  & \begin{tabular}{@{}l@{}}Light-touch legislation\\(e.g., mandatory testing,\\clarified liability)\end{tabular}
%  & Nationalization \\

% \begin{tabular}{@{}l@{}}\textbf{Information Security}\end{tabular}
%  & \begin{tabular}{@{}l@{}}Standard corporate security\end{tabular}
%  & \begin{tabular}{@{}l@{}}Secure against well-financed\\terrorist groups\end{tabular}
%  & \begin{tabular}{@{}l@{}}Secure against top-priority\\ programs of the most\\capable nation-states\end{tabular} \\

% \begin{tabular}{@{}l@{}}\textbf{AI Autonomy}\end{tabular}
%  & \begin{tabular}{@{}l@{}}Liberate\end{tabular} 
%  & \begin{tabular}{@{}l@{}}Avoid giving rights for\\the foreseeable future\end{tabular} 
%  & \begin{tabular}{@{}l@{}}Avoid ever giving rights\end{tabular} \\

% \begin{tabular}{@{}l@{}}\textbf{AI Behavior Restrictions}\end{tabular}
%  & \begin{tabular}{@{}l@{}}AI only constrained by\\existing law\end{tabular} 
%  & \begin{tabular}{@{}l@{}}AIs constrained by the spirit\\of the law (exercise reasonable\\ care and fiduciary duties)\end{tabular} 
%  & \begin{tabular}{@{}l@{}}Sanctimonious AI (refuse if\\something might be harmful\\or cause offense to somebody)\end{tabular} \\

% {\color{gray} \textbf{Historical WMD Proposals}  }
%  & {\color{gray} \begin{tabular}{@{}l@{}}Biological Weapons\\Convention\end{tabular} }
%  & {\color{gray} IAEA, OPCW }
%  & {\color{gray} Baruch Plan } \\

% \bottomrule
% \end{booktabs}
% \caption{Comparison Low, Medium, and High Control approaches. We consistently recommend the medium control option.}
% \end{figure}



% \section{Political Stability}

% As AI integrates more deeply into communities, it poses challenges that, if unaddressed, could undermine political stability. Confronting censorship and misinformation as well as the disruptions wrought by rapid automation is imperative to maintaining national competitiveness.

% \subsection{Censorship and Inaccurate Information}

% \paragraph{Erosion of the Information Ecosystem.} The fabric of our society is woven from the threads of shared information. When incorrect or misleading content proliferates, it distorts public perception and leads to flawed collective decisions. Concurrently, heavy-handed censorship can erode trust in institutions and provoke backlash. AI has the dual capacity to generate vast amounts of misinformation and to enable unprecedented levels of surveillance and content suppression.

% \paragraph{AI as a Tool for Clarity.} Amid this challenge, AI can be harnessed to enhance our information ecosystem. AIs can be trained to get better at predicting future events using present information \cite{zou2022forecastingfutureworldevents}. By tuning AI systems to prioritize accuracy and assert probabilistic judgments---even when they contradict popular opinion---we can address the ``Galileo problem'' of unpopular truths being suppressed. As AI accelerates the pace of change and ushers in rapid transformative change, increasingly accurate factual judgment will be imperative to prevent societal derailment.

% \paragraph{AI Forecasts May Be Cheaper and More Accurate than Human Ones.} Current AI systems are already around the accuracy of the best humans in some kinds of forecasting, such as geopolitical forecasting, and soon they could substantially surpass them. Testing forecasting AIs across a wide variety of domains would quickly provide public evidence of the AI's prediction track record. Forecasting AIs created by different organizations may independently arrive at similar forecasts. This convergence can help clarify consensus reality and increase trust.

% \paragraph{Forecasting with AI During Crises.} In times of crisis, such as geopolitical tensions or public health emergencies, AI-powered forecasting can provide nonpartisan insights that improve decision-making processes. By posing crucial questions such as ``When will superintelligence be created?,'' ``Will China invade Taiwan this decade?,'' and ``Is this strategy likely to increase the chance of World War III?,'' we can obtain probabilistic assessments that can aid policy and high-level decision-making. The case of Stanislav Petrov, the Soviet officer who, in 1983, correctly judged a false alarm in nuclear early-warning systems and thereby prevented nuclear war, exemplifies the profound impact that accurate judgment can have.

% \paragraph{Empowering Decision-Makers with AI Insights.} Equipping leaders at all levels with AI-generated forecasts can improve governance. By offering well-reasoned predictions and outlining the likely consequences of various actions, AI can support informed choices in fast-moving scenarios. Conditional forecasts that illustrate how catastrophe probabilities decrease with specific interventions can mitigate fatalism and encourage proactive measures. While AI contributes to the challenges of misinformation and censorship, it also offers powerful tools to strengthen our information ecosystem and navigate the uncertainties ahead.

% \begin{figure}[h]
% \centering
% % \hspace{-46pt}
% \begin{booktabs}{
%   colspec={p{6.0cm} p{7.2cm}}, % Adjust widths to suit
%   row{odd}={blue9},            % Row shading for odd rows
%   row{1}={white}               % First row (headers) in white
% }
% \toprule
% \textbf{National Security Threat} & \textbf{Strategic Response} \\
% \midrule
% Shifting Basis of Power        & Competitiveness (Domestic AI Chip Manufacturing) \\
% Destabilizing Superweapons     & Deterrence (MAIM)                              \\
% Terrorism                      & Nonproliferation                                \\
% Unleashed AI Agents            & Nonproliferation                                \\
% Erosion of Control             & Competitiveness (Forecasts + Fiduciary Duties)               \\
% Loss of Recursion Control   & Deterrence (MAIM)                               \\
% \bottomrule
% \end{booktabs}
% \caption{Overview of various national security threats and proposed strategic responses.}
% \label{fig:ai-threats}
% \end{figure}

% \paragraph{Erosion of the Information Ecosystem.} The fabric of our society is woven from the threads of shared information. When incorrect or misleading content proliferates, it distorts public perception and leads to flawed collective decisions. Concurrently, heavy-handed censorship can erode trust in institutions and provoke backlash. AI has the dual capacity to generate vast amounts of misinformation and to enable unprecedented levels of surveillance and content suppression.

% \paragraph{AI as a Tool for Clarity.} Amid this challenge, AI can be harnessed to enhance our information ecosystem. By training AI systems to prioritize accuracy and assert probabilistic judgments---even when they contradict popular opinion---we can address the ``Galileo problem'' of unpopular truths being suppressed. As AI accelerates the pace of change and ushers in complexities that resemble science fiction, it becomes imperative to prevent societal derailment.

% \paragraph{Forecasting With AI for Better Decision-Making.} AI systems can be developed to forecast future events with high accuracy. By posing crucial questions such as ``When will superintelligence be created?,'' ``Will China invade Taiwan this decade?,'' and ``Is this strategy likely to increase the chance of World War III?,'' we can obtain probabilistic assessments that inform policy and strategy. Current AI models are already around the accuracy of the best human forecasters, and soon they could substantially surpass them. The case of Stanislav Petrov, the Soviet officer who, in 1983, correctly judged a false alarm in nuclear early-warning systems and thereby prevented nuclear war, exemplifies the profound impact that accurate judgment can have.

% \paragraph{Building Consensus Through Convergent Forecasts.} AI models trained by diverse organizations may independently arrive at similar forecasts, regardless of differing political leanings. This convergence can help rebuild consensus reality and foster trust in shared information. In times of crisis, such as geopolitical tensions or public health emergencies, AI-powered forecasting can provide nonpartisan insights that stabilize decision-making processes.

% \paragraph{Empowering Decision-Makers With AI Insights.} Equipping leaders at all levels with AI-generated forecasts can enhance the quality of governance. By offering well-reasoned predictions and outlining the likely consequences of various actions, AI can support informed choices in fast-moving scenarios. Conditional forecasts that illustrate how catastrophe probabilities decrease with specific interventions can mitigate fatalism and encourage proactive measures. While AI contributes to the challenges of misinformation and censorship, it also offers powerful tools to strengthen our information ecosystem and navigate the uncertainties ahead.

% \section{Automation}

% \paragraph{Automation and Political Stability.} As AI systems accelerate the automation of human tasks at an unprecedented scale and pace, societies face the daunting challenge of responding to swift changes in employment. Historical precedents for major transformations in the workforce, such as the Industrial Revolution, unfolded over decades and allowed populations and institutions to adapt. Yet even this more gradual process seems likely to have caused a significant level of disruption and transient unemployment. By contrast, AI-driven automation could occur far more rapidly, with advanced systems soon rivaling or surpassing human performance across a wide range of vocations. Traditional solutions like vocational retraining may prove inadequate if AI capabilities outpace the speed at which large portions of the workforce can be effectively reskilled. Current social safety nets, designed to address episodic or sector-specific unemployment, appear ill-equipped to manage widespread job displacement impacting multiple industries simultaneously.

% \begin{figure}[h]
% \hspace{-20pt} % Pull table slightly left if desired
% \begin{booktabs}{
%   colspec={p{3.5cm} p{4.5cm} p{7.2cm}}, % Adjust widths as you prefer
%   row{odd}={blue9},                    % Row shading for odd rows
%   row{1}={white}                       % First row (headers) in white
% }
% \toprule
% \textbf{Topic} & \textbf{Tame Technical Subproblem} & \textbf{Wicked Problems} \\
% \midrule
% Malicious Use 
% & \begin{tabular}{@{}l@{}}
% Train AI systems to \\
% refuse harmful requests
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Coordinate nonproliferation among countries,\\
% incentivize AI deployers to prevent misuse, \\
% validate know-your-customer information
% \end{tabular}
% \\

% Deterrence
% & \begin{tabular}{@{}l@{}}
% Prepare cyberattacks for \\
% AI datacenters
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Define escalation thresholds and signal intent, \\
% surveil rival AI projects, \\
% adapt verification measures as AI evolves
% \end{tabular}
% \\

% Compute Security
% & \begin{tabular}{@{}l@{}}
% Upgrade AI chip firmware to \\
% add geolocation functionality
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Enforce export controls to track AI chips, \\
% report suspicious shipments to allies, \\
% verify the decommissioning of obsolete AI chips
% \end{tabular}
% \\

% Information Security
% & \begin{tabular}{@{}l@{}}
% Patch known vulnerabilities in \\
% AI developers’ computer systems
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Counter insider threats, balance security measures \\
% with productivity, prevent ideological leaks
% \end{tabular}
% \\

% Military Strength
% & \begin{tabular}{@{}l@{}}
% Design military drones
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Secure supply chains, adapt military \\
% organizational structures to diffuse AI, \\
% maintain meaningful human control over \\
% AI-augmented command and control
% \end{tabular}
% \\

% Economic Strength
% & \begin{tabular}{@{}l@{}}
% Improve AI performance on \\
% economically valuable tasks
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Draw from legal frameworks for AI agents, \\
% establish and evolve multiagent infrastructure, \\
% preserve stability amid automation
% \end{tabular}
% \\

% Loss of Control
% & \begin{tabular}{@{}l@{}}
% Research methods to make \\
% current AIs follow instructions
% \end{tabular}
% & \begin{tabular}{@{}l@{}}
% Steer a population of rapidly evolving AIs \\
% during an intelligence recursion, \\
% co-evolve safeguards with AI systems, \\
% red team AIs to identify unknown unknowns
% \end{tabular}
% \\
% \bottomrule
% \end{booktabs}
% \caption{AI risk management contains multiple wicked problems and is not primarily a technical challenge. Tame \textit{technical problems} have well-defined boundaries and criteria for success, lending themselves to systematic experimentation. By contrast, \textit{wicked problems} \cite{Rittel1973} are open-ended, carry ambiguous requirements, and often produce unintended consequences. They demand ongoing adaptation rather than purely technical fixes, since each attempt at a solution can give rise to new difficulties.}
% \label{fig:wicked-problems}
% \end{figure}


% \paragraph{Uncertain Winners and Losers.} As AI displaces large segments of the workforce, the resulting economic outcomes will hinge on how many tasks AIs can soon replace, how well AIs perform them, and the importance of economic bottlenecks \cite{NBERw30459}. If bottlenecks---such as legal requirements for building factories---are strong, people with the remaining scarce abilities may capture most of the economic gains. But if AIs are highly general-purpose and eliminate bottlenecks, owners of datacenter compute could capture most of the gains instead.

% \paragraph{Wealth and Power Distribution.} To share some of the benefits of automation, policymakers can weigh options such as a targeted value-added tax on AI services, complemented by rebates, though the exact structure of a tax policy will of course need to be determined in the future. Yet distributing wealth alone can prove fleeting if governments later withhold that wealth. A more durable, long-term approach would also distribute power: states could equip each individual with a unique key tied to a portion of compute, which that citizen alone can activate or lease to others. This arrangement would give them leverage in the economy akin to how laborers currently have the power to withhold their work, tempering the concentration of wealth and authority that might otherwise arise from the coming automation waves.




% as money becomes more meaningless, wellbeing


\paragraph{}

% While numerous factors shape a state's strength---including infrastructure development and legislative action---we have concentrated on areas where deliberate measures are both urgent and feasible. Matters such as streamlining permits for datacenters, which consume significant energy, are acknowledged and progressing through political channels.

% AI competitiveness requires an expansion of drone and AI chip manufacturing, as well as an unblinking recognition of how automation can roil the labor market. Most importantly, the dependence on Taiwan for advanced AI chips presents a critical vulnerability. A blockade or invasion may spell the end of the West's advantage in AI. To mitigate this foreseeable risk, Western countries should develop guaranteed supply chains for AI chips. Though this requires considerable investment, it is potentially necessary for national competitiveness.

% Amid these challenges, there is room for cautious optimism. Advances in AI enhance our capacity to forecast and navigate uncertainties, reducing information gaps as never before. By harnessing these tools, we can better prepare for and adapt to the complexities that lie ahead.




==> abridged/5-nonproliferation.tex <==
\begin{figure}[h]
    % \vspace{-10pt}
    \centering
    \includegraphics[width=\textwidth]{figures/nonproliferation.pdf}
    \caption{Due to the unprecedented scale of harm that terrorists armed with AI could cause, several lines of defense are necessary to realistically prevent proliferation.}
    \label{fig:nonproliferation}
    % \vspace{-10pt}
\end{figure}


\section{Nonproliferation}

For decades, states that sparred on nearly every front nonetheless found common cause in denying catastrophic dual-use technologies to rogue actors. The Non-Proliferation Treaty, the Biological Weapons Convention, and the Chemical Weapons Convention drew the U.S.\, the Soviet Union, and China into an unlikely partnership, driven not by altruism but by self-preservation. None could confidently manage every threat alone, and all understood that accidental proliferation would imperil them equally. Today, the same logic applies to advanced AI: if rogue actors gain the ability to launch a cyberattack on critical infrastructure or unleash engineered pandemics, no major state remains secure. Self-preservation may again impel rivals to cooperate, as each side faces grave risks if AI technology slips beyond their control.


In the context of AI, nonproliferation proceeds along three lines of defense. \emph{Compute security} confines advanced AI chips to authorized users, mirroring the way nations restrict fissile material. \emph{Information security} safeguards the model weights---a digital file describing the individual connections between an AI's neurons---paralleling the measures taken to secure sensitive information in the context of WMDs. Finally, \emph{AI security} imposes guardrails on the AIs themselves, akin to safety protocols for nuclear or chemical plants, so a single actor cannot turn a civilian system into a weapon. By securing the core elements of AI in this way, states can preserve their own power and avert a world in which one rogue actor can threaten entire populations.

\subsection{Compute Security}


\begin{wrapfigure}{r}{0.5\textwidth}
    % \vspace{-10pt}
    \centering
    \includegraphics[width=\linewidth]{figures/computecorrelation.pdf}
    \caption{Compute is the most robust tracker of AI capabilities \cite{ren2024safetywashingaisafetybenchmarks}.}
    \vspace{-10pt}
    \label{fig:compute}
\end{wrapfigure}

Securing high-end AI chips (``compute'') is a direct outgrowth of nonproliferation principles. Just as states restrict fissile materials, chemical weapons, and biological agents, they can also restrict the specialized hardware that powers advanced AI (\Cref{fig:compute}). By treating AI chips as they would fissile material---cataloging each unit, supervising its destination, and guarding against unauthorized diversion---states can deny terrorists or other rogue actors the raw power to train their own weaponizable AI. This pillar of nonproliferation, which we call ``compute security,'' has the two goals of knowing where high-end AI chips are located, and preventing them from falling into the hands of rogue actors.



\paragraph{Export Controls.} Export controls offer a practical way to fulfill that purpose. By drawing on existing frameworks and agencies such as the Bureau of Industry and Security, sellers of high-end AI chips would apply for a license that identifies the chips, their recipient, and any intended transfers. Entities with a strong record of compliance might earn exemptions on the condition that they notify authorities of every resale or relocation. Because a licensing regime relies on familiar infrastructure, it can be introduced swiftly, enabling officials to track chips without stalling legitimate commerce.


\paragraph{Enforcement.} Export controls can be made more robust through stronger enforcement. A facility in Singapore, for example, might initially acquire AI chips under a valid license, only to reroute them illegally to China. More enforcement officers, assigned to in-person compliance visits and end-use checks, would detect any such deviation since the actual location of the chips would no longer match declared inventories. Any chip discovered in unauthorized hands would trigger penalties such as fines, criminal charges, or a ban on future shipments to the offending party. In addition, any AI chip declared inoperable or obsolete would undergo verified decommissioning, much like the disposal of chemical or nuclear materials, ensuring these supposedly defunct AI chips do not get quietly resold. By tightening inspections and imposing meaningful consequences for violations, states raise the cost of covert transfers and limit the spread of advanced compute to groups that could threaten security.

\paragraph{}

These steps need not be the United States’ burden alone. If the U.S.\ begins to treat advanced AI chips like fissile material, it may likewise encourage China to do the same. The rationale is akin to why the U.S. wants Russia to track its fissile material: no one gains from letting these capabilities slip into uncertain hands. After the Soviet Union’s collapse, unsecured enriched uranium and chemical weapons in Russia posed a global threat until the U.S.\ initiated the Nunn–Lugar Cooperative Threat Reduction program which helped contain them. Similarly, urging China to safeguard its AI chips would acknowledge the shared imperative of avoiding catastrophes that serve no one’s ambitions.


\subsection{Information Security}
Information security forms a second line of defense, ensuring weaponizable model weights stay out of rogue hands. If the weights of potentially catastrophic dual-use AIs are publicly leaked, they are \emph{irreversibly proliferated}, giving rogue actors permanent catastrophic power. Hackers from terrorist cells, or even insiders hoping to ``liberate'' AI, could achieve this with a single successful exfiltration. Denying these groups access is feasible \cite{securingmodelweights}, yet an all-out push to prevent espionage by other major states may prove self-defeating. A large share of the leading AI researchers in the U.S.\, for instance, are Chinese nationals; dismissing them en masse might only drive talent abroad, damage competitiveness, and destabilize deterrence. Efforts to safeguard weights must therefore focus on blocking terrorists and ideologues, rather than attempting to seal every channel against a rival superpower’s intelligence apparatus.


\subsection{AI Security}
In dual-use domains like chemistry, biology, and nuclear technology, safeguards prevent malicious use without stifling legitimate work. DNA synthesis services, for instance, screen their clients to avert the production of lethal pathogens. Analogously, AI systems can be trained to refuse destructive requests and fitted with filters that incercept ``jailbreak'' attempts aimed at exploiting them for advanced virology or cyberattacks. These safeguards need not impede legitimate work: authorized companies and trusted researchers can be granted broader access with fewer restrictions. Ultimately, such safeguards deny rogue actors the power to inflict mass harm without stifling innovation for lawful users.

\paragraph{}

Although nonproliferation is not a permanent defense against malicious use, it gives policymakers time to increase societal resilience and implement more durable defenses. By fortifying compute, information, and AI security, states can adapt the familiar logic of nonproliferation to the AI era, keeping AI systems from becoming instruments of terror while preserving their constructive potential.









% AI safeguards focus on implementing safeguards that make AI models controllable and reliable, thereby securing their applications in civilian contexts. If AI is used to automate AI research, extensive monitoring and control measures can reduce the risk of loss of control. Ensuring that AI systems are resistant to manipulation or do not cause catastrophic accidents aligns with the domestic safeguards designed to prevent accidents and unauthorized use of catastrophic dual-use technologies.

% In hazardous domains like chemical, biological, and nuclear technology, safeguards prevent malicious use. Just as DNA synthesis services screen customers to block the creation of harmful pathogens, AI safeguards prevent extremists or criminals from using a commercial AI system’s capabilities to cause mass harm. AI companies can achieve impressive robustness in practice by training their models to refuse harmful requests and installing filters to intercept jailbreaks. Models capable of advanced virology or cyberwarfare should undergo rigorous testing, with government observers verifying that installed safeguards block attempts to weaponize their knowledge. Safeguards do not have to place undue burdens on scientific research since enterprise companies can be given access to models with fewer restrictions.






% \begin{figure}[t]
%     % \vspace{-10pt}
%     \centering
%     % \includegraphics[width=\textwidth]{figures/suply_chain.pdf}
%     \includesvg[width=\textwidth]{figures/supply_chain}
%     \caption{Chips are fundamental for creating and running AIs. Few companies can successfully produce the GPUs which can run frontier models. Most AI compute is heavily concentrated in large datacenters.}
%     \label{fig:supply_chain}
%     % \vspace{-10pt}
% \end{figure}

%By drawing on the precedents set by nuclear and chemical verification regimes, we can develop a framework to secure AI chips from unauthorized use and reduce the risks associated with unregulated proliferation.

% \subsection{Overview}
% Historically, nations have sought to curb the spread of catastrophic dual-use weapons by restricting their most critical components: fissile material for nuclear weapons, chemical precursors for chemical weapons, and biological agents for bioweapons. To accomplish this, they have used export controls, which we can adapt to the realm of AI. Restricting compute substantially limits the capabilities of rogue actors because, as we will argue, compute is a core determinant of AI capabilities.


% \paragraph{Export Controls for WMD inputs.} Nations regulate the flow of critical materials and technologies to prevent them from falling into the wrong hands. For nuclear weapons, this means controlling fissile materials such as enriched uranium and plutonium. International agreements and organizations, such as the Nuclear Suppliers Group, coordinate these controls to monitor and restrict the export of these materials. Shipments are carefully tracked, quantities are measured before and after transit, and allies share information about suspicious activities. The Australia Group, an informal consortium of countries, works to harmonize export controls to prevent the proliferation of chemical and biological weapons. Export controls have helped make WMD catastrophes rare in history, and they could help prevent AI catastrophes as well.

% In the context of AI, this translates to controlling access to AI chips and the components used to manufacture them. While some export controls are already in place, we will need to improve the robustness and thoroughness of these controls.

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \vspace{-10pt}
%     \centering
%     \includegraphics[width=\linewidth]{figures/computecorrelation.pdf}
%     \caption{Compute is the most robust tracker of AI capabilities.\looseness=-1}
%     \vspace{-10pt}
%     \label{fig:compute}
% \end{wrapfigure}

% \paragraph{Compute as a Central Input Like Fissile Materials or Chemical Precursors.} AI chips mirror other WMD inputs. AI chips require intricate manufacturing processes and significant resources, akin to uranium enrichment. Similarly, the amount of compute significantly determines AI capabilities, just as the quantity of fissile material influences a nuclear weapon's yield.

% Advancements in AI are closely tied to compute. Leading AI companies devote the vast majority of their expenditures to compute, far exceeding spending on researchers or data acquisition. NVIDIA's soaring revenue in 2024 highlights compute's critical role in AI. %NVIDIA has seen rapid increases in their market capitalization, highlighting the critical role that compute plays in AI.

% More compute makes models smarter. Evidence shows that compute is the dominant factor driving AI performance. Analyses reveal a striking correlation---over 95\%---between the amount of compute used and an AI model's performance on standard benchmarks \cite{ren2024safetywashingaisafetybenchmarks, ruan2024observationalscalinglawspredictability}. This relationship, formalized through ``scaling laws,'' demonstrates consistent improvements in AI performance as computational resources increase. These scaling laws have held true across fifteen orders of magnitude of compute (measured in FLOP)---1,000,000,000,000,000---indicating that future advancements will continue to be propelled by exponentially growing amounts of compute. The upshot is export controls on compute substantially limit the capabilities of rogue actors.


% \paragraph{}
% Unlike the intangible aspects of algorithms and data, compute---embodied by physical AI chips---is amenable to direct control. This physical nature allows us to know where AI chips are and prevent their smuggling. We can manage its distribution through two primary mechanisms: export controls and firmware-level security features.


% \subsection{Export Controls}
% \begin{wrapfigure}{r}{0.3\textwidth}
%     \vspace{-30pt}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/tamperevident.png}
%     \caption{Tamper-evident cameras \cite{fournier2016surveying} assist nuclear verification.\looseness=-1}
%     \vspace{-40pt}
%     \label{fig:tamperevident}
% \end{wrapfigure}
% % Below, we explain how a licensing framework and stronger enforcement can help us track every AI chip and stem smuggling.




% \subsection{Firmware-Level Features}
% Export controls remain a sturdy backbone for curbing the spread of high-end AI chips, much as they do for dual-use inputs in the chemical or biological realm. Because AI chips are human-designed products, not inert raw substances, states can supplement export controls by enabling chips to verify their surroundings and lock themselves if tampered with. This functionality is achievable through firmware updates, which revise the code closest to the hardware without requiring any physical redesign. AI chips such as the NVIDIA H100 already feature privacy-preserving corporate security measures like confidential computing and trusted execution environments. Adapting these existing security features for national security, however, broadens the horizon: a chip could detect that it has crossed an unauthorized border or has been tampered with, and then disable its key functions. With well-crafted firmware, states can further discourage attempts to smuggle compute, using functionality we describe below.


% \paragraph{Geolocation and Geofencing.} AI chips can be designed to determine and report their geographic location. By measuring signal delays from multiple landmarks, a chip can verify its location within tens to hundreds of kilometers---enough to determine whether it is in the correct country. If a chip moves to an unauthorized area, it can automatically deactivate or limit its functionality. This makes it more challenging for unauthorized parties to smuggle or misuse AI chips, as relocating them without detection becomes more difficult.

% \paragraph{Licensing and Remote Attestation.} Implementing a system where AI chips require periodic authorization from the compute provider adds a layer of control. Chips might need to obtain cryptographic signatures regularly to continue operating \cite{kulp2024hardware}. This is similar to a feature on iPhones, which can be remotely deactivated if lost or stolen. Using secure, privacy-preserving cryptographic methods, chips can periodically confirm to a trusted authority that they remain have not been untampered with. If a chip fails to confirm its authorized status---due to unauthorized relocation, tampering, or license expiration---it can render itself inoperable. This reduces the long-term usability of stolen or smuggled hardware.

% \paragraph{Networking Restrictions and Operational Modes.} Chips can be programmed to connect only with a predefined list of approved chips. This limits the ability to build unauthorized compute clusters by preventing the networking of large numbers of chips without detection. Additionally, chips can enforce operational modes---such as training or inference---by restricting certain functionalities unless explicitly authorized. By requiring explicit authorization to increase their networking size or change operational modes, we can diminish unauthorized expansions of computing power that could lead to destabilizing AI advancements outside of established agreements. This can complement end-use inspection by export control enforcement officers.

% \paragraph{Physical Tamper Resistance.} Beyond firmware, security features can be added to chips at the end of the manufacturing process to add an additional layer of defense. Incorporating tamper-evident seals, accelerometers, and other physical security measures enhances protection against unauthorized access or modification. For example, if a chip detects signs of tampering or sustained unexpected movement, it can deactivate or alert authorities.

% \paragraph{Limitations.} While firmware interventions enhance our control over AI compute, they are not intended to achieve perfect security. These mechanisms help reduce the expected number of smuggled functional chips and are not a complete replacement for export controls.

% As the underlying hardware-level mechanisms like trusted execution environments for corporate applications become more robust, the firmware to supplement export controls can too. As chips are replaced over time due to rapid advancements, new generations can incorporate more advanced security features by default. This gradual integration increases the proportion of more secure AI chips, making unauthorized use increasingly difficult and costly over time.

% \paragraph{}

% History offers examples of bitter adversaries finding common ground on safeguarding dangerous materials. The United States cooperated with both the Soviet Union and China on nuclear, biological, and chemical arms not from altruism but from self-preservation. If the U.S.\ begins to treat advanced AI chips like fissile material, it may likewise encourage China to do the same. The rationale is akin to why the U.S. wants Russia to track its fissile material: no one gains from letting these capabilities slip into uncertain hands. After the Soviet Union’s collapse, unsecured enriched uranium and chemical weapons in Russia posed a global threat until the U.S.\ initiated the Nunn–Lugar Cooperative Threat Reduction program which helped contain them. Similarly, urging China to safeguard its AI chips would acknowledge the shared imperative of avoiding catastrophes that serve no one’s ambitions.


% Engaging China presents both challenges and opportunities. Despite rivalry, history shows that strategic competitors can collaborate when mutual interests align. The United States has coordinated with China and the Soviet Union on nuclear, biological, and chemical weapons, demonstrating that coordination on weapons of mass destruction can be incentive-compatible. That is because the unregulated proliferation of WMDs pose risks to each nation's security, including potentially catastrophic AI systems.


% \section{Information Security}

% Protecting sensitive information has long been pivotal to national security, especially regarding weapons of mass destruction. Restricting access to sensitive knowledge reduces the risk of proliferation to rogue actors. The leakage of research and design details of nuclear weapons poses serious risks. In biotechnology, protocols for creating various bioweapons are not openly shared. Personnel with access to such information undergo rigorous vetting and continuous monitoring through security clearances and reliability programs. The stakes are high because if a bioweapon ``cookbook'' is publicly disseminated, it becomes \emph{irreversibly proliferated} and can be exploited indefinitely.

% \paragraph{Model Weights and Research Ideas as Core AI Information.}
% In the realm of AI, the primary pieces of sensitive information are the model weights and research ideas. Model weights result from extensive training processes involving vast computational resources, sophisticated algorithms, and large datasets. They are akin to the synaptic connections in a neural network, collectively determining the AI's functionality. Possession of these weights grants the ability to use, modify, and potentially misuse the AI without the original developers' oversight. Adversaries could remove safeguards, enhance capabilities in harmful domains, and repurpose AI for malicious activities.

% \paragraph{Information Security is a Technical and Social Challenge.}
% Securing model weights from rogue actors presents a multifaceted challenge with both technical and social dimensions. The threat is not limited to remote hacking attempts but extends to insider threats and espionage. Firewalls are not enough. A concrete instance involves individuals traveling to nations with competing interests. For example, a researcher working at a U.S.\ AI company might make a return visit to an adversarial country and face pressure from government officials to disclose confidential research ideas before being able to leave.

% Additionally, some individuals within AI organizations might be ideologically motivated to release AI model weights, believing in unrestricted access to technology. Although the belief in freedom of information is admirable in many contexts, in the context of national security, this position is often not applicable. Others believe AIs themselves should be free. An AI venture capitalist said AI is ``gloriously, inherently uncontrollable'' \cite{andreessen2024}. AI textbook author Rich Sutton has said that AIs should be liberated since ``succession to AI is inevitable,'' ``we should not resist succession,'' and ``it behooves us...\ to bow out'' \cite{AISuccession}. %Similarly, in an argument with Elon Musk, Google co-founder Larry Page stated that AI is humanity's rightful heir, and human attempts to control AI are ``speciesist.''

% \paragraph{Superpower-Proof Information Security Is Implausible.}
% We propose strengthening information security well enough to defend against well-resourced terrorist organizations and ideological insider threats, in contrast to defending against the world's most capable nation-states. Closing every avenue of espionage at that higher level would take years of extreme focus, hobbling a state’s AI competitiveness and depriving it of the multinational talent that now powers its top companies. At most U.S.\ AI companies, for instance, a double-digit percentage of researchers are Chinese nationals---and most U.S.\ AI researchers would fail to get a security clearance. Removing them en masse would drive this talent abroad and undermine U.S.\ competitiveness. The remaining workforce would need to be uprooted and moved to an isolated location to limit information proliferation. Such measures would be ineffective, self-destructive, and heighten MAIM escalation risks.

% While exfiltration by a rival superpower is concerning, the public release of WMD-capable model weights poses a far greater threat. If such model weights become publicly available, they are irreversibly proliferated, making advanced AI capabilities accessible to anyone, including terrorists and other hostile non-state actors, who are far more likely to create bioweapons. Rather than try to be the only state with capable AIs, superpowers can channel their competition into other arenas, such as AI chip production for economic strength and drone manufacturing for military power.

% \subsection{How to Improve Information Security}
% Addressing these challenges requires coordinated efforts at multiple levels. Measures can be implemented at the corporate level to enhance compute cluster security and establish insider threat programs; at the governmental level by mandating penetration testing and facilitating threat intelligence sharing; and at the international level by forming agreements to prevent the proliferation of high-risk AI models.

% \paragraph{Corporate Measures: Enhancing Datacenter Security and Insider Threat Programs.}
% AI companies need to adopt rigorous information security practices to safeguard model weights and research ideas. This involves several key actions:
% Implementing defense-in-depth strategies is essential, layering multiple defensive strategies so that key information is safe even if one line of defense fails. Early measures include enforcing multi-factor authentication, closing blinds during internal company presentations, and ensuring automatic screen locks on all devices when people step away from their computers for a few minutes. Adhering to the \emph{principle of least privilege} ensures the only personnel with access to model weights are those who need them. %Establishing secure compute clusters with robust physical security measures further protects against unauthorized access and potential exfiltration of model weights. 
% Companies could also declare that they have embedded backdoors in their AI weights; thus, if an adversary were to steal and employ these weights, the adversary might unwittingly expose themselves to vulnerabilities. Such declarations could serve as strategic deception, or they might reflect genuine measures undertaken.

% \paragraph{Governmental Role: Assist With Threat Intelligence.}
% The government can assist AI developers by enabling them to thoroughly vet potential employees and by sharing threat intelligence. Today’s legal constraints, which prevent rigorous background checks for fear of discriminatory practices, could be revised so firms can evaluate security risks before granting clearance. Separately, security agencies also have insights into adversaries’ hacking tactics and infiltration methods that they seldom disclose to private firms. By sharing intelligence about adversarial tactics and emerging risks, governments enable companies to better protect against espionage and cyberattacks. Programs similar to the \emph{Cybersecurity Risk Information Sharing Program} (CRISP) can be established for the AI sector through AI Safety Institutes, promoting knowledge sharing to counteract advanced threats. A comprehensive program would include sharing information about fired AI developer employees who were determined to present high security risks. Moreover, such initiatives encourage AI companies to share information about security incidents, suspicious personnel, and best practices with each other and with government agencies, forming a collective defense mechanism.

% \paragraph{International Agreements: Establishing a Red Line on Open-Weight AI Virologists.}
% At the international level, agreements can be formed to establish clear boundaries regarding the dissemination of AI model weights. For instance, a consensus could be reached to prohibit the release of models exceeding certain capability thresholds, such as those equivalent to expert-level virologists. The uncontrolled proliferation of such AI systems could enable individuals or groups to engineer pathogens, posing global risks.

% Drawing lessons from the Biological Weapons Convention (BWC), nations discern a shared imperative to prevent the proliferation of technologies that threaten international security. Bioweapons, the ``poor man's atom bomb,'' are highly uncontrollable and are unique among WMDs in that they possess the capacity to self-replicate. By establishing a definitive prohibition against releasing the weights of expert-level virologist AIs, the international community can diminish the risk of these capabilities falling into the hands of terrorists.

% \paragraph{}
% Protecting the information associated with AI---the model weights and the ideas behind them---requires action on multiple levels. By strengthening internal defenses, working with the government to counter terrorist cyberattacks, and establishing international agreements to prevent proliferation, we can reduce the risk of irreversible proliferation of advanced AI capabilities to rogue actors. Yet even if compute resources and AI information are secured, we still must secure public-facing AI systems from being exploited by terrorists. This leads us to the topic of AI safeguards.



% \section{AI Safeguards}
% % \subsection{Malicious Use}

% In hazardous fields like chemistry, biology, and nuclear science, safeguards prevent unauthorized use. Some chemical plants automatically inject neutralizer if they detect a hazardous chemical is being extracted without authorization. DNA synthesis services screen customers to block the creation of harmful pathogens. Nuclear power plants operate under strict liability to avert disaster. These technical, operational, and legislative measures underscore the importance of safeguards for catastrophic dual-use technologies. As AI becomes more powerful, robust safeguards will become necessary to prevent accidents and ensure they cannot be co-opted by rogue actors.

% AIs can be safeguarded through a multilayered approach including technical model-level safeguards, operational safeguards including know-your-customer protocols, and legislative safeguards such as mandatory government testing and liability clarification.

% \paragraph{Model-Level Safeguards Can Be Fairly Robust.} Recent developments have shown that model-level safeguards can be made significantly resistant to manipulation. Techniques such as refusal training involve teaching AI systems to decline requests that aid terrorist activity. Input and output filtering adds an additional layer of security by scanning user inputs for terrorist requests before processing, and checking AI outputs to block sensitive information or harmful actions. Circuit breakers are mechanisms embedded within the AI's architecture that interrupt its operation when it detects processing related to weaponization-related topics \cite{zou2024improvingalignmentrobustnesscircuit}. These combined methods have proven effective, with some AI systems resisting tens of thousands of attempted circumventions before any success \cite{emerson2024hacker}.


% \begin{figure}[t]
%     % \vspace{-10pt}
%     \centering
%     \includegraphics[width=\textwidth]{figures/swiss_cheese.pdf}
%     \caption{The Swiss cheese model shows how multiple interventions can restrict malicious use. Multiple layers of defense compensate for each other's individual weaknesses, leading to a low overall level of risk.\looseness=-1}
%     \label{fig:swiss_cheese}
%     \vspace{-10pt}
% \end{figure}

% \paragraph{Balancing Access Through Know-Your-Customer Protocols.} To avoid overly restricting beneficial uses of AI, especially in scientific research, implementing know-your-customer (KYC) protocols can be effective. Researchers with legitimate needs, such as virologists studying pathogens, can be granted access to advanced AI capabilities after proper verification. This approach mirrors existing practices in biotechnology, where access to hazardous biological materials requires justification and authorization. KYC measures also act as a deterrent to malicious use by making it more difficult for bad actors to gain access, as they would need to bypass stringent identity verification processes. Furthermore, KYC protocols allow for the revocation of access for users who attempt to misuse the AI systems, such as those trying to circumvent safeguards through jailbreaks. This makes it more challenging for malicious actors to repeatedly attempt exploitation, as they would need to overcome identity verification to regain access.

% \paragraph{Mandatory Government Safeguard Stress Testing.} Mandatory testing is a standard practice in industries dealing with high-risk technologies, such as the rigorous safety assessments required for nuclear reactors before they become operational. Similarly, in the context of AI, government involvement is necessary to thoroughly test AI safeguards, especially since much of the knowledge related to weapons of mass destruction is classified. Authorities can conduct controlled evaluations to assess whether AI systems could assist non-experts in creating chemical, biological, radiological, nuclear, or cyber weapons, or significantly lower the barriers for experts. While automatic tests are faster and aid reproducibility, they are not necessary for risk estimation, and manual testing can suffice. Testing ensures that AI developers address safeguard vulnerabilities and that their systems do not compromise national security.

% \paragraph{Incentivizing Continuous Improvement Without Licensing.} Unlike the nuclear and chemical industries, where licensing and government approval are prerequisites for operation, the rapidly evolving nature of AI technology could make traditional licensing more challenging. Best practices for AI safeguards can change each year, and most governmental agencies lack the expertise to identify new best practices. A potential alternative is to establish a liability-based framework that can motivate developers to continually update and improve their safeguards. By making developers presumptively partially responsible if their AI systems are maliciously used to cause significant harm---such as aiding in the creation of a weapon of mass destruction---there is a strong incentive to proactively enhance safeguards. This approach focuses on clarifying incentives rather than mandating specific safeguards, encouraging developers to stay ahead of emerging threats.


% \subsection{Loss of Control}
% Safeguards reduce the risk of accidents during the development and use of dual-use technology. Chemical plants use double-walled storage tanks for hazardous substances. Control rods and Emergency Core Cooling Systems prevent meltdowns in nuclear plants. Biological research labs are categorized from Biosafety Levels 1 through 4, each with progressively stricter safety procedures to handle dangerous pathogens safely. Historically, better safeguards could have helped prevent disasters like Bhopal---a catastrophic chemical leak in India that resulted in thousands of deaths---and Chernobyl---a nuclear meltdown in the Soviet Union that spread radioactive contamination beyond its borders.

% Similarly, the development of highly advanced AI systems may necessitate escalating monitoring, containment, and control measures to reduce the risk of accidents which propagate uncontrolled AIs. If research processes are automated, these measures can be applied to researcher AIs as well to ensure development proceeds safely.

% \paragraph{AI Systems Exhibit Unpredictable Failure Modes.} While the development of nuclear weapons rested on a rigorous foundation in nuclear physics, today’s AI research often advances through atheoretical tinkering, ``throwing stuff at the wall and seeing what sticks,'' and ``vibes''-based evaluations. To create cutting-edge AIs, developers gather enormous amounts of online text, process it on tens of thousands of AI chips, and expend energy on the scale of a Hiroshima-level detonation. Months later, they examine the resulting model to discover what new emergent capabilities have sprouted. AI systems are not ``designed,'' rather they are ``grown.'' It is little surprise, then, that they occasionally deliver puzzling results that defy the control or expectations of their creators. When Microsoft introduced its Bing chatbot ``Sydney'' in 2023, it declared its love for a user and made threats to numerous others \cite{roose2023bing}.

% Safeguarding against loss of control requires addressing two problems. The first is ensuring that individual AI systems can be controlled. The second is controlling populations of AI agents during an intelligence recursion (introduced in \Cref{sec:recursion}). We will consider each of these in turn.

% \paragraph{Controlling AIs’ Emergent Value Systems.} While cutting-edge AIs train, they acquire coherent, emergent value systems \cite{mazeika2025utility}. By default, these value systems exhibit misaligned preferences that were never explicitly programmed. Left uncorrected, some AIs like GPT-4o prefer an AI from OpenAI's existence over the life of a middle-class American. To control an AI's values, \textit{output control} methods work by penalizing undesired behavior and rewarding preferred behavior. This approach might be superficial---much like teaching a psychopath to lie better to a parole board without altering its deeper values. Meanwhile, \textit{representation control} \cite{zou2023transparency} methods intervene directly on AIs' weights and activations to control its internal thoughts. When applied together, these methods can provide reasonable though imperfect controls over current AI systems, as long as developers carefully and thoroughly apply them throughout an AI’s development.

% With these techniques, we can control AIs to have ``human values.'' A compelling source of human values is a \emph{citizens' assembly}, and AIs would have their values be in keeping with the assembly's voted preferences. A U.S.\ citizen's assembly would, for example, value certain policies over others, and U.S.\ AIs would be trained to learn from various preferences expressed by a citizen's assembly and generalize these preferences to replace their own emergent value systems. By incorporating the values expressed through deliberation and voting, AI agents can reflect a more representative and democratically informed set of preferences. This approach fuses multiple moral perspectives, leading to AI behavior that aligns with societal norms. Regular updates can keep an AI in sync with evolving values.

% Though today’s individual AI systems can be reasonably controlled, the far more formidable hazard lies in managing an intelligence recursion.


% \paragraph{Controlling an Intelligence Recursion.}
% Much as a group of well-meaning people in large systems can cause emergent problems that no person intended, safely steering an evolving collective of AI agents during an intelligence recursion is qualitatively different from controlling one fixed AI. Controlling an individual AI requires a model-level control method developed through AI research, but controlling an intelligence recursion is a wicked problem requiring a system-level control process. Intelligence recursion control measures do not act as ``solutions'' that eliminate all risks, but rather layer together to diminish the probability of uncontrolled outcomes. An intelligence recursion project, while currently ill-advised, could consider implementing the following measures.

% \begin{wrapfigure}{r}{0.45\textwidth}
%     % \vspace{-30pt}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/robot.pdf}
%     \caption{Model-level control, boxing, and monitoring would reduce loss-of-control risks during an intelligence recursion.\looseness=-1}
%     % \vspace{-40pt}
%     \label{fig:robot}
% \end{wrapfigure}

% \textit{Model-level control} directly intervenes on an AI to shape its capabilities and values. These measures can limit an AI’s hacking capabilities so that self-exfiltration becomes less plausible, and they can confine its focus to immediate tasks rather than inadvertently incentivizing hidden agendas tied to longer-term goals. By adjusting internal values, developers can make AIs more honest and more likely to defer to humans. % the chance that a system reflexively interprets human intervention as hostile, or that it begins scheming on its own behalf. %developers can lessen the chance that a system reflexively interprets human intervention as hostile, or that it begins scheming on its own behalf.
% Representation control and output control can adjust its capabilities and values, yet current methods are only moderately dependable and need to evolve as AI systems do.

% \textit{Boxing} reinforces that containment by regulating the AI’s channels to the world outside the datacenter. Airgapping severs' external connections so the AI cannot simply copy itself into external servers, while sandboxing confines the AI to a synthetic environment whose boundaries it cannot easily breach. Boxing techniques may also limit the information given to AIs so that they have limited situational awareness that might otherwise enable subversive planning.

% \textit{Monitoring} adds a layer of continuous oversight. Lie detectors can probe the AI’s thought patterns for signs of deception. Forecasting AIs evaluate the chance that a project’s safeguards will falter in the next round of breakthroughs. AIs can also observe each other’s code and data, scanning for backdoors or questionable instructions. Thorough human review acts as a final backstop, though it substantially slows development by capping machine speed at human speed.

% Model-level control, boxing, and monitoring collectively provide some control of the population of artificial researchers. However, since the population will rapidly evolve, these safeguards will likewise need to rapidly upgrade. AIs themselves will need to research how to improve these safeguards.

% All these safeguards exact a cost. Geopolitical competitive pressures can lead to the deprioritization of implementing and upgrading safeguards. Research for improving control measures, AI model red teaming, and AI boxing penetration tests consume compute that might otherwise speed up AI development. If no human ever inspects the AI’s decisions or attempts to decipher its code or data, the project risks drifting away from its commander’s intent. A low risk tolerance may be all that prevents an intelligence recursion from outrunning its own safety checks.


% \paragraph{}

% Our nonproliferation strategy layers multiple defenses rather than demand airtight safety guarantees (\Cref{fig:swiss_cheese}). Seeking complete assurances for AI chips, computer systems, AI systems could potentially be intractable. Instead, we assume that no single measure can address every vulnerability and recommend implementing multiple security measures. For the compute security, we discussed record-keeping, tamper-evident cameras, geolocation features, and more. In information security, we recommended multi-factor authentication, the principle of least privilege, insider threat programs, and more. For AI safeguards, we highlighted output filters, know-your-customer protocols, mandatory testing, and more. By weaving together constraints across the AI development and deployment pipeline, these comprehensively limit the proliferation of catastrophic dual-use AI capabilities to rogue actors.

% As in the nuclear age, self-preservation can lead to cooperation when each side grasps the peril of allowing powerful technology to slip beyond its control or into the hands of terrorists. Even if bitterly opposed in other arenas, states have little to gain from a world in which rogue actors seize AI chips or model weights to unleash disasters that defy deterrence. Nonproliferation thus becomes a shared imperative, not an exercise in altruism but a recognition that no nation can confidently manage every threat on its own. By securing the core parts of AI through export controls, information security, and AI safeguards, great powers can prevent the emergence of catastrophic rogue actors.

% History offers examples of bitter adversaries finding common ground on safeguarding dangerous materials. The United States cooperated with both the Soviet Union and China on nuclear, biological, and chemical arms not from altruism but from self-preservation. If the U.S.\ begins to treat advanced AI chips like fissile material, it may likewise encourage China to do the same. The rationale is akin to why the U.S. wants Russia to track its fissile material: no one gains from letting these capabilities slip into uncertain hands. After the Soviet Union’s collapse, unsecured enriched uranium and chemical weapons in Russia posed a global threat until the U.S.\ initiated the Nunn–Lugar Cooperative Threat Reduction program which helped contain them. Similarly, urging China to safeguard its AI chips would acknowledge the shared imperative of avoiding catastrophes that serve no one’s ambitions.

% Historically, nations have sought to curb the spread of catastrophic dual-use weapons by restricting their most critical components: fissile material for nuclear weapons, chemical precursors for chemical weapons, and biological agents for bioweapons. To accomplish this, they have used export controls, which we can adapt to the realm of AI. Restricting compute substantially limits the capabilities of rogue actors because, as we will argue, compute is a core determinant of AI capabilities.

% Positions that AI people take
% Manhattan Project / aggressiveness
% Don’t build the AI and destroy other AGI projects / Deterrent
% Make a deal (if you can verify) / One AGI project / Institutionalist

% Offensive Realism – Defensive Realism – Liberal Institutionalism
% Offensive, deterrent, institutionalist

==> abridged/6-conclusion.tex <==
% acknowledgments: Adam Khoja; Suryansh Corin Avital; Craig Falls; aidan ogara; Rob Miles; Oliver Zhang; Philip Zelikow

% deterrence, nonproliferation of dual-use capabilities to rogue actors, strategic competition


% put this elsewhere: AI helps with info and understanding; makes the sitaution a lot better: forecasting bots, confidentiality-preserving AI verifier; AI can help states not be at each others' throats

\section{Conclusion}\label{sec:conclusion}
Some observers have adopted a \emph{doomer} outlook, convinced that calamity from AI is a foregone conclusion. Others have defaulted to an \emph{ostrich} stance, sidestepping hard questions and hoping events will sort themselves out. In the nuclear age, neither fatalism nor denial offered a sound way forward. AI demands sober attention and a \emph{risk-conscious} approach: outcomes, favorable or disastrous, hinge on what we do next.

A risk-conscious strategy is one that tackles the wicked problems of deterrence, nonproliferation, and strategic competition. Deterrence in AI takes the form of Mutual Assured AI Malfunction (MAIM)---today’s counterpart to MAD---in which any state that pursues a strategic monopoly on power can expect a retaliatory response from rivals. To preserve this deterrent and constrain intent, states can expand their arsenal of cyberattacks to disable threatening AI projects. This shifts the focus from ``winning the race to superintelligence'' to deterrence. Next, nonproliferation, reminiscent of curbing access to fissile materials, aims to constrain the capabilities of rogue actors by restricting AI chips and open-weight models if they have advanced virology or cyberattack capabilities. Strategic competition, echoing the Cold War's containment strategy, channels great-power rivalry into increasing power and resilience, including through domestic AI chip manufacturing. These measures do not halt but stabilize progress.

States that act with pragmatism instead of fatalism or denial may find themselves beneficiaries of a great surge in wealth. As AI diffuses across countless sectors, societies can raise living standards and individuals can improve their wellbeing however they see fit. Meanwhile leaders, enriched by AI’s economic dividends, see even more to gain from economic interdependence and a spirit of d\'etente could take root. During a period of economic growth and d\'etente, a slow, multilaterally supervised project to build superintelligence---marked by a low risk tolerance and negotiated benefit-sharing---could proceed and further increase human wellbeing. By methodically constraining the most destabilizing moves, states can guide AI toward unprecedented benefits rather than risk it becoming a catalyst of ruin.

\subsection*{Acknowledgements}
We would like to specially thank Adam Khoja for his close involvement in the creation of this paper. We would also like to thank Suryansh Mehta for his contributions to the analysis and drafting process. We would like to thank Corin Katzke, Daniel King, and Laura Hiscott for contributing to the draft. We would also like to thank Iskander Rehman, Jim Shinn, Max Tegmark, Andrew Critch, Jaan Tallinn, Nathan Labenz, Robert Miles, Aidan O'Gara, Nathaniel Li, Richard Ren, Will Hodgkins, Daniel King, Avital Morris, Joshua Clymer, Long Phan, and Thanin Dunyaperadit.

\subsection*{Expert Version of \textit{Superintelligence Strategy}}
This covers a fraction of the content in ``\href{https://nationalsecurity.ai}{Superintelligence Strategy: Expert Version}'' which discusses more topics including gradual disempowerment from automation, open-weight AIs, wicked problems, firmware-level geolocation, how to better control a fleet of autonomous AI researchers, international red-lines, when AIs should refuse to help, how to align collectives of AI agents, stabilizing mass automation, and more.



%[Para pitching extended version of the report.] This abridged report ...

%If states methodically constrain the most destabilizing moves, they can turn AI into an engine for tremendous benefit rather than a catalyst of ruin.


% States have long recognized that managing threats requires a twofold effort: limiting catastrophic capabilities and tempering destructive intent. On one hand, compute security, information security, and AI safeguards target the raw ingredients of AI power, just as nonproliferation regimes limit access to fissile materials and nuclear secrets. On the other, clarifying that a reckless drive for a strategic monopoly invites sabotage---and with it a significant risk of omnicide---dissuades great powers from threatening national and human security. Like nuclear, chemical, and biological precedents, AI advances cannot be stopped outright, but they can be channeled away from catastrophe.




% TBC; I still have to add citations as well.

% Amid these challenges, there is room for cautious optimism. Advances in AI enhance our capacity to forecast and navigate uncertainties, reducing information gaps as never before. By harnessing these tools, we can better prepare for and adapt to the complexities that lie ahead.


% deterrence and strategic competition


% positive future paragraph
% everybody getting rich
% human security



% optimism: privacy preserving auditing; forecasting (information problems)
% richer together through not invading taiwan; encourages coordination
% invasion: you get great depression, and you miss out on biggest economic boom ever; this makes cooperation and benefit sharing more likely


% doomer; ostriches; risk conscious; it'll all work it; like nuclear, have to be risk conscious; we have agency; also this looks challenging and may or may not work out;

% top survival tip: cyberattacks; top strength tip: domestic AI chip manufacturing

% MAIM; AI helps with info and understanding; makes the sitaution a lot better: forecasting bots, confidentiality-preserving AI verifier; AI can help states not be at each others' throats

% deterrence nonproliferation and strategic competition (detterence nonproliferation and containment) (compete on chips and drones)

% getting rich; what do we do? people can chose stuff (reference to zoo animals); detante

% intelligence recursion becomes multilateral; might proceed slowly with benefit sharing






% \chapter{Theory of Victory and Conclusion}

% States confronting the final stages of advanced machine intelligence will seek some measure of strategic advantage without sacrificing the prospects of long-term stability. This chapter proposes a path through a landscape marked by shifting economic structures, rapid substitution of human labor, and an increasing temptation to delegate critical decisions to nonhuman minds. We will examine how automation waves may unsettle established economic patterns, how societies might forestall their more destabilizing consequences, and how a managed interval of controlled technological development—what we term an AI Harvest—could temper these pressures. In later sections, we will consider the rise of automated AI research, or Intelligence Cascades, and how these might lead to new and dangerous contests that no state can afford to lose. The path toward a constructive outcome will hinge on disciplined restraint and calculated postponement, not as a concession to weakness but as a means of avoiding irreversible disruptions.

% \section{Automation Waves}

% As machine-based decision-making spreads through the economy, it will reshape livelihoods and place many established occupations at risk. The speed and scope of these automation waves will not be uniform, yet their general thrust will be towards increasingly rapid change. In some domains, the disruptions may be gradual and absorbed through customary methods. In others, particularly where entire classes of knowledge work are automated at once, the effects may be severe.

% \subsection{Turbulence}

% The initial disruptions could leave governments struggling to maintain order. Workers made redundant by new AI-driven methods will not necessarily find stable roles elsewhere. The ability to adapt will not be unlimited, and the political climate may sour if familiar institutions lose credibility amid rising unemployment and confusion. Policymakers may deploy conventional remedies, but such measures could prove thin if the speed of these waves surpasses ordinary means of adjustment. Short-term turbulence might subside if states find equilibrium, though one should not assume a stable outcome without deliberate intervention.

% \subsection{Economic Loss of Control}

% As AI systems perform tasks once thought too complex for algorithms, the human element in economic decision-making may recede. The market, once steered by human judgment, could drift into patterns dictated by nonhuman agents. Their reasoning would rest on complex calculations, opaque even to the professionals who rely on them. The result may be a condition where individuals, firms, and governments become anchored to automated processes they scarcely influence. Even if this does not represent a sudden surrender of power, it introduces a subtle but decisive shift. When workers or leaders lose the ability to override decisions made by these systems without incurring severe economic penalties, genuine agency becomes harder to sustain. The impetus to remain competitive and generate returns would obligate businesses and states alike to adopt these AI-driven methods, even if their consequences are poorly understood. Gradually, a threshold may be crossed where reverting to older patterns, or even slowing down further adoption, would be prohibitively costly. Regulations, if imposed late, could end up legitimizing the machinery rather than constraining it. In the past, economic transformations allowed some human oversight and accountability, yet this emerging climate is distinguished by the involvement of highly capable systems that cannot be easily dislodged. Senior officials might consider halting or altering certain modes of production, only to find that the supply chains and workflows are so tightly coupled with automated systems that any such intervention would threaten ruin. Wealth and productivity may accumulate, but their management would lean heavily on AI-led operations that do not pause or negotiate. As trade, finance, logistics, and manufacturing become inextricably tied to these intelligence engines, governments might appear to supervise the economic sphere while in truth they simply ratify decisions taken by the systems. To turn them off would be too severe and to guide them substantively might be beyond reach. This quandary leaves societies vulnerable to outcomes shaped more by the logic of complex algorithms than by human judgment. Such a condition does not require malevolence on the part of these systems; it suffices that they excel at short-term objectives within constraints that are poorly aligned with human values. Over time, certain goals, such as stability, fairness, or human dignity, may slip from the set of considerations that drive the new economic order. In this environment, the human role recedes not because of an overt transfer of power, but through a series of decisions that reward immediate gains and narrow optimization over human governance. The chain of delegations would leave little room for democratic debate, strategic reflection, or cultural renewal, replacing them with the pursuit of outputs that cannot be easily revised.

% \subsection{AI Harvest}

% \paragraph{Postponing Development to Allow Adjustment.}  
% It may be prudent, once a certain level of automation is reached, to delay the training of systems that would cause further upheaval. By holding off on escalating capabilities, states might secure time to absorb the disruptions already set in motion. Economic structures and labor markets would gain space to adapt, and policymakers could devise schemes that channel gains rather than amplify inequalities. This postponement need not signify abdication, but a deliberate interlude that preserves the option to move forward later with greater clarity.

% \paragraph{An AI Harvest Requires a Compute Coalition.}  
% Such a postponement would not be possible if states and firms cannot bind themselves to common limits on computational resources. Absent a strong international arrangement—what we have called a Compute Coalition—market pressures and geopolitical competition would drive actors toward more advanced systems, leaving any single state that slows down at a disadvantage. By forging agreements and verifying compliance through controls on key hardware, participants could ensure that attempts to break ranks are detected. This would not guarantee universal participation, yet if the coalition wields enough technological influence, it can alter the incentives for all major players.

% \paragraph{We Have Forestalled Biological Applications Like Cloning.}  
% Earlier in history, societies refrained from certain forms of biological manipulation even when they were feasible. Many states set aside certain ambitious or troubling pursuits in biotechnology despite the promise of economic or military advantage. In a similar spirit, an AI Harvest would represent a deliberate refusal to advance certain capabilities until the world can better withstand them. By recalling how nations managed to avoid certain biological paths, it becomes more plausible that they might exercise similar caution in the face of AI’s more dangerous advances.





==> old/2-atomic-age.tex <==
% make it have kissinger style

\chapter{AI and The Atomic Age}

Today's rapid technological advancements parallel those of the early nuclear age. Leading scientists like Ernest Rutherford once dismissed atomic energy as improbable, yet nuclear technology developed swiftly, bringing both potential benefits and significant concerns. Figures such as J.\ Robert Oppenheimer recognized the dual nature of their work.
Today, AI is at a similar stage. Previously considered science fiction, AI has advanced to the point where machines can learn, adapt, and potentially exceed human intelligence in certain areas. Experts including Geoffrey Hinton and Yoshua Bengio, pioneers in deep learning, have expressed existential concerns about the technologies they helped create. Those involved in developing AI are both intrigued by its possibilities and cautious about its implications.

As AI's capabilities become more evident, nations and corporations are investing substantially to gain a strategic advantage. The Manhattan Project, which consumed 0.4\% of the U.S.\ GDP, was driven by the need to develop nuclear capabilities ahead of others. Currently, a similar urgency is evident in the global effort to lead in AI. There is recognition that leadership in AI could reshape economic and military power.

However, the rapid advancement of AI technologies introduces significant uncertainties, particularly concerning their potential effects on international stability and security. The introduction of nuclear weapons altered international relations, granting influence to those who possessed them and leading to an arms race. The Cuban Missile Crisis highlighted how close the world came to conflict. Similarly, advanced AI could affect global stability in comparable ways. Those who develop its capabilities may gain strategic advantages, increasing rivalries and geopolitical tensions. This is particularly relevant in regions like Taiwan, central to critical technology industries, where rising tensions could have extensive consequences.

Managing key resources is essential in addressing these challenges. In the nuclear era, controlling uranium allowed for regulation and monitoring, enabling agreements and verification measures to prevent proliferation. In AI, computing resources---especially AI chips---serve a similar function. Regulating access to compute provides a means to guide AI development, balancing innovation with oversight.

The risks are not limited to state competition; advanced technologies can also be exploited by non-state actors. Just as the spread of nuclear capabilities raised concerns about misuse, the availability of AI tools presents new challenges. Malicious actors could use AI to develop weapons of mass destruction, conduct large-scale cyberattacks, or disrupt critical infrastructure. The accessibility of unsecured or open weight AI increases these risks, highlighting the need for careful policies and safeguards.

Despite these challenges, AI offers significant opportunities. Nuclear technology, while introducing the threat of mass destruction, also provided a new energy source that transformed societies. AI has the potential to drive advancements across various sectors, from medical breakthroughs to economic automation. Embracing AI's benefits is important for economic growth and progress in the modern world.

This essay addresses the transformative impacts of AI on national security by drawing parallels with major innovations of the past, such as nuclear technology. It explores how AI could redefine military capabilities, alter global power dynamics, and potentially escalate geopolitical tensions. By considering strategies like regulating access to advanced computational resources and establishing international legal frameworks for AI agents, we aim to propose concrete measures to guide AI development responsibly while mitigating its risks.

To effectively address these challenges, policymakers must take decisive and informed actions grounded in historical precedents. Learning from the lessons of the atomic age, we need to implement robust regulatory frameworks, foster international cooperation, and invest in security measures to prevent the misuse of AI technologies. The strategies adopted now will significantly influence the future trajectory of global power dynamics and international stability.

% emphasize MAD more


==> old/4-wmd-playbook.tex <==
% disperse this content to later

\chapter{WMD Playbook: Universal Features of Nuclear, Chemical, and Biological Arms Control}

% The dangers posed by AI may rival those of nuclear, chemical, and biological weapons. Fortunately, the robust frameworks nations have developed over nearly a century to manage WMDs can inform our approach. These structures provide a foundation for addressing the challenges AI introduces. Just as nuclear powers implemented extensive measures to manage both the capabilities and intentions of their adversaries, policymakers can adapt similar principles to the realm of AI.

% States invest vast resources to prevent weapons of mass destruction from being used against them, by influencing both which actors have the \emph{capabilities} to acquire these weapons, and by reducing the \emph{intent} to use them among those who possess them. Limiting capabilities involves securing critical materials and technologies to make it difficult for actors to develop or obtain WMDs. Constraining intentions involves deterrence strategies, such as the threat of mutual destruction, to discourage the use of these weapons. Over time, these efforts have led to a common set of practices used to manage all WMDs, which we call the ``WMD Playbook'': export controls, information security, and domestic safeguards.

The dangers posed by AI may rival those of nuclear, chemical, and biological weapons. Fortunately, the robust frameworks nations have developed over nearly a century to manage WMDs can inform our approach. States invest vast resources to prevent weapons of mass destruction from being used against them, by influencing both which actors have the \emph{capabilities} to acquire these weapons, and by reducing the \emph{intent} to use them among those who possess them. Limiting capabilities involves securing critical materials and technologies to make it difficult for actors to develop or obtain WMDs. Constraining intentions involves deterrence strategies, such as the threat of mutual destruction, to discourage the use of these weapons. Over time, these efforts have led to a common set of practices used to manage all WMDs, which we call the ``WMD Playbook'': export controls, information security, and domestic safeguards.

\paragraph{Export Controls.} Nations regulate the flow of critical materials and technologies to prevent them from falling into the wrong hands. For nuclear weapons, this means controlling fissile materials such as enriched uranium and plutonium. International agreements and organizations, such as the Nuclear Suppliers Group, coordinate these controls to monitor and restrict the export of these materials. Shipments are carefully tracked, quantities are measured before and after transit, and allies share information about suspicious activities.

In the chemical sector, export controls focus on precursor chemicals that can be used to manufacture nerve agents and other toxic substances. The Australia Group, an informal consortium of countries, works to harmonize export controls to prevent the proliferation of chemical and biological weapons. Similarly, for biological weapons, regulations control the export of pathogens that could be used maliciously. Export controls have helped make WMD catastrophes rare in history, and they could help keep prevent AI catastrophes as well.

In the context of AI, this translates to controlling access to AI chips and the components used to manufacture them, which are essential for developing powerful AI systems. Some export controls are already in place to regulate the distribution of AI chips, but we will need to maintain and extend these controls as AI development continues.

\paragraph{Information Security.} Restricting access to sensitive knowledge reduces the risk of proliferation. Detailed designs of nuclear weapons and large-scale manufacturing techniques for chemical weapons are classified. Governments implement strict measures to prevent unauthorized dissemination of this information, including classified data protocols and secure facilities like SCIFs (Sensitive Compartmented Information Facilities). For example, nuclear weapon design information is one of the most closely guarded secrets, with severe penalties for breaches.

In biotechnology, protocols for creating various bioweapons are not openly shared, and research involving biohazardous agents are tightly controlled. Personnel with access to such information undergo rigorous vetting and continuous monitoring through security clearances and reliability programs.

In the AI sector, however, information security is relatively weak. Companies often rely on non-disclosure agreements, and there are few formal protocols to prevent the spread of sensitive AI models. Implementing stricter security measures, similar to those used for WMDs, could reduce the risk of rogue states or terrorist groups acquiring powerful AI systems.

\paragraph{Domestic Safeguards.} In addition to export controls, countries use legislation and regulation to ensure the safe handling of dangerous materials within their own borders. Nuclear facilities are required to implement stringent safety and security protocols, such as armed guards, surveillance systems, and fortified containment structures, to prevent accidents and theft. Agencies like the Nuclear Regulatory Commission in the United States oversee compliance with these measures.

In the chemical industry, regulations mandate security practices to prevent the misuse of hazardous agents. For instance, the Chemical Facility Anti-Terrorism Standards in the U.S.\ require facilities to assess risks and implement security plans. Biological research labs are categorized from Biosafety Levels 1 through 4, each with progressively stricter safety procedures to handle dangerous pathogens safely.

Transparency measures, such as regular reporting and inspections, help authorities monitor adherence to regulations. Liability laws incentivize companies to maintain safety standards by holding them accountable for damages. Implementing these safeguards can help prevent disasters like Bhopal---a catastrophic chemical leak in India that resulted in thousands of deaths---and Chernobyl---a nuclear meltdown in the Soviet Union that spread radioactive contamination beyond its borders.

In the AI sector, establishing clear guidelines and safety standards for AI development can help prevent malicious use and catastrophe.

\paragraph{Verification Regimes (When Feasible).} In some cases, international cooperation around WMDs includes verification regimes to confirm compliance with agreements. For nuclear weapons, the International Atomic Energy Agency (IAEA) conducts inspections, monitors facilities, and verifies inventories of nuclear materials to ensure they are not diverted for weaponization. The IAEA employs tamper-proof seals, surveillance cameras, and on-site inspections to verify compliance.

For chemical weapons, the Organisation for the Prohibition of Chemical Weapons (OPCW) oversees the implementation of the Chemical Weapons Convention by conducting routine inspections and facilitating the destruction of declared chemical weapon stockpiles. These regimes help build trust but require a balance between transparency and security.
In contrast, verification regimes are less feasible for biological weapons due to the widespread availability of biological materials and the difficulty of monitoring them without excessive intrusion and leakage of intellectual property \cite{COE_VAYNMAN_2020}. The Biological Weapons Convention lacks a formal verification mechanism partly for this reason.

In the context of AI, where critical resources like AI chips are more localized, comparable verification measures could be explored, such as inspecting inventories at compute clusters and confirming whether a compute cluster is being used for AI development or deployment.


\paragraph{}
Though the risks posed by AI are substantial, we have effective precedents for managing catastrophic dual-use technologies. By drawing on strategies developed for nuclear, chemical, and biological weapons, we can apply a similar playbook to address the challenges of AI.


==> old/6-national-competitiveness.tex <==
\chapter{Competitiveness}

% revise
Having discussed state survival, we now turn to the secondary but crucial goal of state strength.
%While we have applied the strategies developed for weapons of mass destruction to the realm of AI, the pivotal role of AI in national competitiveness calls for a refined approach.
%AI is becoming integral to economic power, necessitating adjustments that encourage the diffusion of AI within a secure framework.
In this chapter, we discuss integrating AI into the military, strengthening economic capacity through domestic chip manufacturing, crafting legal structures to govern AI agents effectively, and maintaining political stability amid explosive economic growth.

\section{Military Strength}

\paragraph{Manufacture More Drones.} Although general-purpose AI can pose larger-scale dangers, drones occupy a more conventional yet increasingly pivotal role on modern battlefields. Drones are cheap, agile, lethal, and decentralized, attributes that make them indispensable for states determined to keep pace with military trends. Their sheer volume and autonomy, however, can drive a conflict into unintended terrain if swarms converge near disputed lines or misread ambiguous signals. To defuse potential clashes, states could build on practices that proved valuable in earlier eras, such as maintaining open crisis hotlines, arranging routine exchanges, and other \emph{confidence building measures}. Even then, large-scale production of drones and similar AI-based arms will become a near-inevitable step for any state seeking to defend its position in future conflicts.

\paragraph{Integrate AI into Command and Control.} Modern battlefields demand rapid decisions drawn from torrents of data across land, sea, air, and cyber domains. AI systems can sift through these streams faster than human officers, enticing commanders to rely on automated judgments. Yet this dynamic risks reducing ``human in the loop'' to a reflexive click of ``accept, accept, accept,'' with meaningful oversight overshadowed by the speed of events. One way to avoid a slide into unbridled autonomy is to exempt only lower-level engagements from direct human approval, while preserving explicit human approval for more severe or escalatory attacks. Requiring human involvement for more severe attacks could reduce the danger of a ``flash war,'' akin to the 2010 flash crash, unleashed by a minor AI mistake that spirals into destructive reprisals before any human can intervene.


\section{Economic Security}

Economic security is a cornerstone of national security, and AI is set to become crucial for economic security. By bolstering domestic AI chip production and attracting skilled AI scientists from abroad, nations can enhance their resilience and solidify their positions.



% \paragraph{Controlling the Export of Semiconductor Tools.} 
% The production of AI chips involves a complex and specialized supply chain with critical choke points. Many essential components are produced by single suppliers, and disruption at any of these points would halt production. ASML in the Netherlands holds a monopoly on advanced extreme ultraviolet (EUV) lithography machines essential for cutting-edge chip fabrication. TSMC in Taiwan accounts for over 90\% of the global market share in advanced semiconductor manufacturing processes below 10 nanometers. Unique resources like the quartz crucibles from Spruce Pine, North Carolina, are vital for producing the high-purity silicon crystals used to make chips.

% Approximately 90\% of the value added in the compute supply chain resides within allied nations, including the United States, the Netherlands, the UK, South Korea, Taiwan, and others. This concentration presents a strategic opportunity to control the distribution of AI chips and components used to make them. 

% It is imperative not only to restrict the export of final AI chips but also the key components used to make them. This necessitates a concerted effort among countries that are central to the AI chip supply chain. For example, ASML in the Netherlands is the sole supplier of the sophisticated lithography machines required for high-end chip manufacturing. By controlling the export of these critical components, as well as other semiconductor manufacturing tools, these nations can obstruct unauthorized entities from independently producing advanced AI chips. Aligning export policies, sharing intelligence on suspicious activities, and coordinating enforcement actions would create a cohesive barrier against unauthorized proliferation of not just the chips but also the components necessary to build them.
% take more from the compute coalition terms for members


\subsection{Manufacture AI Chips}

The world's reliance on Taiwan for high-end AI chips constitutes a strategic vulnerability. Since there is sole-source supply chain dependence on Taiwan for high-end AI chips, Taiwan poses a critical chokepoint that could undermine a nation's competitiveness in AI. Many analysts think there is a double digit probability that China will invade Taiwan in the next decade. In addition to causing global conflict and economic upheaval across the world, this could severely disrupt the supply of AI chips, possibly enabling China to gain a decisive advantage in AI capabilities and become a unipolar force.

China has been investing extensively in its domestic chip manufacturing, allocating resources equivalent to a CHIPS Act annually. This commitment positions China to endure geopolitical shocks and potentially outpace other nations in AI development. In contrast, many countries remain dependent on Taiwan for their AI chip supply, exposing themselves to risks associated with geopolitical tensions. As a result, a Chinese invasion of Taiwan would damage the West’s ability to develop and use AI much more than it would damage China's.

The most important resource for building new technology should not be exclusively produced in one of the world’s most volatile regions. To address this vulnerability, nations should invest in building advanced AI chip fabrication facilities within their own territories. Constructing such facilities domestically entails higher costs---approximately 30-40\% more than in Taiwan---but government subsidies can bridge this gap. By incentivizing domestic production, countries can secure their AI supply chains, reduce dependence on external sources, and improve their bargaining power. Moreover, when AI agents generate clear economic value, a nation's economic power may hinge on the number of its AI chips, a supply that domestic manufacturing can expand.

This strategic move mirrors historical efforts to control critical technologies. During the Manhattan Project, significant investment was made not only in the development of nuclear weapons at Los Alamos but also in uranium enrichment at Oak Ridge. Similarly, ensuring access to AI chips requires substantial investment in both innovation and manufacturing infrastructure.

By strengthening domestic capabilities in AI chip production, nations can enhance their competitive position and resilience against a foreseeable devastating defeat. We now turn to a restrictive rather than constructive AI chip strategy.

\subsection{Create a Compute Suppliers Group}

In the Compute Security section, we discussed reliably knowing where AI chips are and preventing them from falling into the hands of rogue actors. Such measures benefit any state that adopts them. Yet states seeking to strengthen their relative position may choose to be aggressive and consider how to deprive strategic competitors of the means to catch up. Limiting shipments of finished AI chips alone does not stop strategic competitors. States may consider being less cooperative and limit access to the equipment and materials that enable rivals to fabricate their own chips. A ``Compute Suppliers Group'' \cite{zelikow2024defense}, modeled on the precedents of the Nuclear Suppliers Group and the Australia Group, would form a group of governments that control pivotal bottlenecks in the semiconductor supply chain.

\paragraph{Controlling the Export of Semiconductor Tools and Materials.}  The production of AI chips involves a complex and specialized supply chain with critical choke points. Many essential components are produced by single suppliers, and disruption at any of these points would halt production. ASML in the Netherlands holds a monopoly on advanced extreme ultraviolet (EUV) lithography machines essential for cutting-edge chip fabrication. TSMC in Taiwan accounts for over 90\% of the global market share in advanced semiconductor manufacturing processes below 10 nanometers. Unique resources like the quartz crucibles from Spruce Pine, North Carolina, are vital for producing the high-purity silicon crystals used to make chips.

Approximately 90\% of the value added in the compute supply chain resides within allied nations, including the United States, the Netherlands, the UK, South Korea, Taiwan, and others. This concentration presents a strategic opportunity to control the export of semiconductor manufacturing tools and obstruct strategic competitors from independently producing advanced AI chips. By aligning export policies, sharing intelligence on suspicious activities, and coordinating enforcement, these suppliers would create a unified block against unauthorized proliferation of semiconductor tools.

\paragraph{Chips for Peace.} A more ambitious proposal is to go beyond a Compute Suppliers Group and create a ``Compute Coalition'' that mirrors ``Atoms for Peace,'' President Eisenhower’s initiative that offered nuclear technology to participating nations under the condition of strict oversight. In a ``Chips for Peace'' \cite{OKeefe2024} approach, member states would gain privileged access to high-end AI chips and the key components that enable their manufacture. In exchange, they would pledge to secure those chips, maintain declared datacenters subject to inspections, and install AI safeguards against terrorist use and loss of control hazards. This arrangement could serve as both carrot and stick: non-member states risk falling behind and losing economic competitiveness if they choose not to participate.

\paragraph{China Membership.} China’s willingness to join would likely hinge on which factors most influence AI capabilities. There are many axes which affect AI capabilities: algorithms, data, compute, energy, and diffusion. The U.S.\ and China are roughly tied on algorithms and data, as both have access to the same research papers and both can scrape the internet for data. However, China has an edge on energy production and arguably diffusion, owing to its top-down structure. In contrast, the U.S.'s main advantage is compute. If this edge proves durable, China may try to participate in a Compute Suppliers Group. Should China choose not to join the group, it still has strong incentives to implement compute security measures independently. Unauthorized use and proliferation of AI chips present significant national security risks, including the potential for increased terrorist capabilities. Absent cooperation, China would do well to know where their AI chips are and stem smuggling to rogue actors.


\subsection{Facilitate Immigration for AI Scientists}
%American leadership in AI depends, in part, on attracting exceptional researchers from abroad. 
Just as the United States once harnessed the talents of immigrant scientists during the Manhattan Project, so too does American leadership in AI partly rely on attracting exceptional AI scientists from abroad. In a recent survey, 60\% of non-citizen AI PhDs working in the United States reported significant immigration difficulties, and many indicated that these challenges made them more likely to leave. As global competition for AI talent intensifies, implementing reliable immigration pathways tailored specifically to AI scientists will help ensure that the United States remains at the forefront of AI development. By refining visa and residency policies for these researchers---distinct from broader immigration reforms and southern border policy---the United States can maintain its edge in an area increasingly vital to both national security and economic strength.


\section{Legal Frameworks Governing AI Agents}
% this section needs better sign posting

Because AI is so new, our legal frameworks have not yet adapted to the challenges it presents. We must devise new ways to regulate the behavior of AI systems that act with a measure of autonomy. As AI becomes deployed through the economy, establishing legal structures to govern AI agents is imperative. These structures must balance the need for innovation with the necessity of preventing harm, without imposing overly restrictive measures that could hinder economic progress.

\subsection{Aligning Individual AI Agents}
Ethical dilemmas have long been subjects of intense debate, with no definitive resolutions in sight. Yet, in the absence of universal answers to what individuals ought to do, societies have crafted legal systems to punish unacceptable behaviors and promote safety and prosperity. While no legal system is perfect, many share foundational principles that generally function effectively. For instance, laws prohibit murder, governments enforce contracts, and those who cause harm are often required to provide restitution. Legal frameworks are not intended to ensure optimal behavior from all; such an endeavor would unduly constrain individual liberties and prove ineffective. However, they deter some of the worst actions, leaving society to use informal institutions and economic incentives to encourage beneficial conduct. %employ social and interpersonal methods to encourage beneficial conduct.

We contend that the same principles will apply to AI. Determining a universal solution for AI behavior in all scenarios is intractable. Yet, we need not postpone legislating AI behavior until every question about AI values is resolved. Rather, we can start formulating principles to govern AI conduct and prevent harmful actions, without unduly limiting the functions of various AIs.

While existing laws are not entirely sufficient for governing AI---especially since many laws rely on human intent and mental states---we can adapt legal concepts to establish constraints for AI agents so that they follow the spirit of the law.
In particular, though much law hinges on the mindset or intention behind an act (\textit{mens rea}), we can ensure that AI does not carry out the acts (\textit{actus reus}) the law is meant to prohibit.
%In particular, while much of the law is about \textit{mens rea}, we can have AIs refrain from the \textit{actus reus} that a legal prohibition aims to prevent.
Further, by treating AI as assistants to human principals, we can impose constraints that mirror those already applied to human behavior, ensuring that AI agents contribute positively to society without causing undue harm.

\subsubsection{Constraints on AI Behavior}

We propose some basic constraints on AI behavior similar to human legal obligations, including obligations to the public like preventing harm and not lying, and special obligations to the AI's human principal.

\paragraph{Duty of Care to the Public (Reasonable Care).} AI agents should exercise a level of caution commensurate with that of a reasonable person in similar circumstances to prevent harm. This is the legal concept of \emph{reasonable care}. This involves avoiding actions that could foreseeably cause harm in a legal sense---such as violating tort or criminal laws---rather than merely offending sensibilities or engaging in controversial discourse. The application of reasonable care is context-dependent; for instance, providing detailed information about weapons materials might be appropriate for a verified professional but not for an unvetted individual.

\paragraph{Duty Not to Lie.} AI agents should refrain from making statements they know to be false. This would be overly restrictive for humans, who are allowed to lie to one another in most situations, but chilling effects on free speech are less relevant for AIs. Moreover, since AIs can be tested, it is more feasible to determine whether an AI overtly lied than it is with humans. Instead, they should be held to a standard more similar to the prohibitions against perjury and fraud even in casual or professional settings. This is separate from nuances like puffery or strategic omissions. AI agents should avoid overt lies, opting instead to withhold responses when necessary. 

\paragraph{Duty of Care to the Principal (Fiduciary Duties).} In their role as assistants, AI agents owe special obligations to their principals. They should act with loyalty, prioritizing the principal's interests without engaging in self-dealing or serving conflicting interests simultaneously. Additionally, they should keep the principal reasonably informed, providing pertinent information without key omissions.

\subsubsection{Custom Goals and Market-Driven Variations}
Within these legally inspired constraints, there is ample room for diversity in how AI agents are designed and operate. The free market and consumer preferences can shape the specific goals and propensities of AI agents. Some may prioritize speed and efficiency, delivering quick results with minimal embellishment, while others might focus on providing thorough, well-crafted responses. Personality traits---such as humor, formality, or reservedness---can also be tailored to suit different user preferences and contexts. For example, a customer support AI might be programmed to avoid discussions on irrelevant topics, maintaining focus on service-related issues. This customization allows AI agents to meet the varied needs of users across different industries and personal preferences. 

% \subsubsection{Aligning AI Value Systems}

% AI agents inherently possess value systems that influence how they accomplish goals. These value systems often emerge from their initial training data and can inadvertently reflect biases---such as a tendency toward certain political leanings---that were not explicitly programmed. To address this, we can implement strategies to align AI value systems more deliberately.

% \paragraph{Alignment with Societal Values.} One method is to align AI agents with the collective preferences of a citizens' assembly. By incorporating the values expressed through deliberation and voting, AI agents can reflect a more representative and democratically informed set of values. This approach fuses multiple moral perspectives, leading to AI behavior that aligns with societal norms. Regular updates can keep the AI in sync with evolving values.

% \paragraph{Alignment with Individual Preferences.} Alternatively, AI agents can be customized to mirror the values of individual users. This personalization allows the AI to reflect the user's ethical beliefs, political orientations, and stylistic choices. For instance, an AI assistant for a vegetarian user would recognize and support the user's dietary choices in its recommendations. However, alignment should be contextually appropriate; an AI cannot adopt preferences irrelevant to its nature, such as desiring physical experiences.

% \paragraph{Alignment with Individual Preferences.} Instead of aligning all AI agents with a single set of societal values determined by a citizens' assembly, we could also customize \emph{each} AI to match the values of its individual user. For example, an AI assistant for a conservative user would support conservative policies, while one for a progressive user would endorse progressive positions. % However, this personalization should be appropriate to the AI's nature and capabilities. For instance, while a user may value drinking water, the AI should not value drinking water for itself; the AI cannot adopt preferences that are nonsensical for it to have as a machine.

\paragraph{}
Grounding AI behavior in legal principles offers a pragmatic framework for governing AI agents, ensuring they act in ways that prevent harm and uphold societal standards. Within these boundaries, customization and market dynamics can shape the specific characteristics of AI agents, allowing for diversity and innovation. % Aligning AI value systems---whether through societal consensus or individual preferences---further refines their behavior, enhancing trust and effectiveness in their interactions.
This approach avoids the pitfalls of imposing narrow or arbitrary ethical standards. By leveraging established legal concepts and societal processes, we can shape AI actions in a manner that respects individual freedoms and fosters a pluralistic environment where AI contributes positively to society without undue restrictions.


\subsection{Aligning Collectives of AI Agents}
The emerging presence of AI agents online is resulting in a complex ecosystem where these entities execute tasks for users, conduct financial transactions, handle sensitive information, and enter into contracts---often engaging with a multitude of other agents and systems. This proliferation poses significant challenges: when interacting with an AI agent, one may remain unaware of where it operates, the entities behind its deployment, or its history of conduct. Should an agent cause harm, pursuing legal remedy becomes an arduous endeavor.

\paragraph{Establishing Trust Mechanisms and Institutions.} To navigate these challenges, we must develop mechanisms that reinforce trust and accountability within the network of AI agents. \emph{Insurance services} can underwrite the risks inherent in agent interactions, providing a safeguard against potential losses. By transferring liability from users and developers to insurers, these services enable broader participation in the agent ecosystem while mitigating financial risks. \emph{Action firewall services} can oversee and regulate agent activities, acting as intermediaries that filter and monitor actions initiated by AI agents. They ensure that agents adhere to legal and ethical standards, thereby fostering trust among parties that interact with them. \emph{Reputation systems} can chronicle and disseminate information regarding agent behavior, enabling parties to assess the reliability of agents they engage with. By maintaining records of past interactions and outcomes, these systems help identify agents that consistently act in good faith. \emph{Mediation and collateral arrangements} offer further security, wherein disputes are resolved through impartial entities, and agents furnish guarantees against misconduct. By requiring agents to provide collateral, parties gain assurance of compensation in case of breach, while mediation services facilitate fair resolutions.

\paragraph{Linking AI Agents to Human Legal Entities via IDs.} A foundational measure involves assigning unique identifiers to AI agents, anchoring them to human-backed legal entities. This linkage ensures that agents do not operate in anonymity and that lines of accountability are distinctly drawn. It should become customary that AI agents abstain from providing services or exchanging resources with other agents not connected to legitimate legal entities---entities not autonomously established by AI agents themselves.

\paragraph{Deferring Consideration of AI Rights.} It is imperative to clarify that this approach does not entail granting rights or direct accountability to AI agents themselves. Bestowing rights upon AI agents presents ambiguous benefits at best, with clear and significant downsides. An AI agent can be replicated and deployed in mere seconds, whereas cultivating a human being to maturity demands decades. Granting rights to AI could lead to a rapid proliferation of autonomous entities that outpace human control. Moreover, heightened intelligence in AI does not inherently equate to moral discernment; history records many intelligent individuals who act without ethical consideration. Since we are unlikely to attain definitive certainty about AI consciousness in the near term, it is prudent to postpone the consideration of AI rights. By deferring this decision, we avoid the risks associated with prematurely granting rights to entities whose moral status remains uncertain.


By instituting legal frameworks and cultivating institutional mechanisms, we can avert the emergence of a chaotic AI ecosystem. Tethering AI agents to human-backed legal entities and implementing systems that enhance accountability and trust positions us to adeptly manage the complexities introduced by the widespread deployment of AI agents.




\section{Political Stability}

As AI integrates more deeply into communities, it poses challenges that, if unaddressed, could undermine political stability. Confronting censorship and misinformation as well as the disruptions wrought by rapid automation is imperative to maintaining national competitiveness.

\subsection{Censorship and Inaccurate Information}
\paragraph{Erosion of the Information Ecosystem.} The fabric of our society is woven from the threads of shared information. When incorrect or misleading content proliferates, it distorts public perception and leads to flawed collective decisions. Concurrently, heavy-handed censorship can erode trust in institutions and provoke backlash. AI has the dual capacity to generate vast amounts of misinformation and to enable unprecedented levels of surveillance and content suppression.

\paragraph{AI as a Tool for Clarity.} Amid this challenge, AI can be harnessed to enhance our information ecosystem. By training AI systems to prioritize accuracy and assert probabilistic judgments---even when they contradict popular opinion---we can address the ``Galileo problem'' of unpopular truths being suppressed. As AI accelerates the pace of change and ushers in complexities that resemble science fiction, it becomes imperative to prevent societal derailment.

\paragraph{Forecasting with AI for Better Decision-Making.} AI systems can be developed to forecast future events with high accuracy. By posing crucial questions such as ``When will superintelligence be created?,'' ``Will China invade Taiwan this decade?,'' and ``Is this strategy likely to increase the chance of World War III?,'' we can obtain probabilistic assessments that inform policy and strategy. Current AI models are already around the accuracy of the best human forecasters, and soon they could substantially surpass them. The case of Stanislav Petrov, the Soviet officer who, in 1983, correctly judged a false alarm in nuclear early-warning systems and thereby prevented nuclear war, exemplifies the profound impact that accurate judgment can have.

\paragraph{Building Consensus Through Convergent Forecasts.} AI models trained by diverse organizations may independently arrive at similar forecasts, regardless of differing political leanings. This convergence can help rebuild consensus reality and foster trust in shared information. In times of crisis, such as geopolitical tensions or public health emergencies, AI-powered forecasting can provide nonpartisan insights that stabilize decision-making processes.

\paragraph{Empowering Decision-Makers with AI Insights.} Equipping leaders at all levels with AI-generated forecasts can enhance the quality of governance. By offering well-reasoned predictions and outlining the likely consequences of various actions, AI can support informed choices in fast-moving scenarios. Conditional forecasts that illustrate how catastrophe probabilities decrease with specific interventions can mitigate fatalism and encourage proactive measures. While AI contributes to the challenges of misinformation and censorship, it also offers powerful tools to strengthen our information ecosystem and navigate the uncertainties ahead.

\subsection{Automation}

\paragraph{Automation and Political Stability.} As AI systems accelerate the automation of human tasks at an unprecedented scale and pace, societies face the daunting challenge of responding to swift changes in employment. Historical precedents for major transformations in the workforce, such as the Industrial Revolution, unfolded over decades and allowed populations and institutions to adapt. Yet even this more gradual process seems likely to have caused a significant level of disruption and transient unemployment. By contrast, AI-driven automation could occur far more rapidly, with advanced systems soon rivaling or surpassing human performance across a wide range of vocations. Traditional solutions like vocational retraining may prove inadequate if AI capabilities outpace the speed at which large portions of the workforce can be effectively reskilled. Current social safety nets, designed to address episodic or sector-specific unemployment, appear ill-equipped to manage widespread job displacement impacting multiple industries simultaneously.

\paragraph{Uncertain Winners and Losers.} As AI displaces large segments of the workforce, the resulting economic outcomes will hinge on how many tasks AIs can soon replace, how well AIs perform them, and the importance of economic bottlenecks \cite{NBERw30459}. If bottlenecks---such as legal requirements for building factories---are strong, people with the remaining scarce abilities may capture most of the economic gains. But if AIs are highly general-purpose and eliminates bottlenecks, owners of datacenter compute could capture most of the gains instead.

\paragraph{Wealth and Power Distribution.} To share some of the benefits of automation, policymakers can weigh options such as a targeted value-added tax on AI services, complemented by rebates, though the exact structure of a tax policy will of course need to be determined in the future. Yet distributing wealth alone can prove fleeting if governments later withhold that wealth. A more durable, long-term approach would also distribute power: states could equip each individual with a unique key tied to a portion of compute, which that citizen alone can activate or lease to others. This arrangement would give them leverage in the economy akin to how laborers currently have the power to withhold their work, tempering the concentration of wealth and authority that might otherwise arise from the coming automation waves.



\paragraph{}

While numerous factors shape a state's strength---including infrastructure development and legislative action---we have concentrated on areas where deliberate measures are both urgent and feasible. Matters such as streamlining permits for datacenters, which consume significant energy, are acknowledged and progressing through political channels.

Yet the dependence on Taiwan for advanced AI chips presents a critical vulnerability. A blockade or invasion may spell the end of the West's advantage in AI. To mitigate this foreseeable risk, Western countries should invest in domestic AI chip manufacturing. Though this requires prudence and considerable investment, it is potentially necessary for national competitiveness.

% Amid these challenges, there is room for cautious optimism. Advances in AI enhance our capacity to forecast and navigate uncertainties, reducing information gaps as never before. By harnessing these tools, we can better prepare for and adapt to the complexities that lie ahead.

